An Alternating Rank-K Nonnegative Least Squares Framework (ARkNLS) for Nonnegative Matrix Factorization

Nonnegative matrix factorization (NMF) is a prominent technique for data dimensionality reduction that has been widely used for text mining, computer vision, pattern discovery, and bioinformatics. In this paper, a framework called ARkNLS (Alternating Rank-k Nonnegativity constrained Least Squares) is proposed for computing NMF. First, a recursive formula for the solution of the rank-k nonnegativity-constrained least squares (NLS) is established. This recursive formula can be used to derive the closed-form solution for the Rank-k NLS problem for any integer k $\ge$ 1. As a result, each subproblem for an alternating rank-k nonnegative least squares framework can be obtained based on this closed form solution. Assuming that all matrices involved in rank-k NLS in the context of NMF computation are of full rank, two of the currently best NMF algorithms HALS (hierarchical alternating least squares) and ANLS-BPP (Alternating NLS based on Block Principal Pivoting) can be considered as special cases of ARkNLS with k = 1 and k = r for rank r NMF, respectively. This paper is then focused on the framework with k = 3, which leads to a new algorithm for NMF via the closed-form solution of the rank-3 NLS problem. Furthermore, a new strategy that efficiently overcomes the potential singularity problem in rank-3 NLS within the context of NMF computation is also presented. Extensive numerical comparisons using real and synthetic data sets demonstrate that the proposed algorithm provides state-of-the-art performance in terms of computational accuracy and cpu time.

==> bibitems_copy.tex <==
\begin{thebibliography}{00}

\bibitem{AG}{\sc A. Shun Ang, and N. Gillis}, {\it Accelerating nonnegative matrix factorization algorithms using extrapolation},
          arXiv:1805.06604v2, 2018.

\bibitem{B}{\sc I. Buciu}, {\it Non-negative matrix factorization, a new tool for feature extraction: Theory and applications},
          Int. J. Computers, Comm. and Control, pp. 67--74, 2008.


\bibitem{BJ}{\sc R. Bro, and S. Jong}, {\it A fast non-negativity-constrained least squares algorithm}, J. Chemom., pp. 393--401, 1997.

\bibitem{BK}{\sc M.H. Van Benthem, and M.R. Keenan}, {\it Fast algorithm for the solution of large-scale non-negativity constrained
           least squares problems}, J. Chemom., pp. 441--450, 2004.

\bibitem{BSJJZ}{\sc T. Bouwmans, A. Sobral, S. Javed, S. K. Jung, and E. Zahzah}, {\it Decomposition into low-rank plus additive
           matrices for background/foreground separation: A review for a comparative evaluation with a large-scale dataset},
           Comp. Sci. Rev., pp. 1--71, 2017.

\bibitem{BTGM}{\sc J. Brunet, P. Tamayo, T. Golub, and J. Mesirov}, {\it Metagenes and molecular pattern discovery
           using matrix factorization}, Proc. Natal. Acad. Sci., pp. 4164--4169, 2004.

\bibitem{CLD}{\sc G. Cui, X. Li, and Y. Dong}, {\it Subspace clustering guided convex nonnegative matrix factorization},
              Neurocomputing,  pp. 38--48, 2018.

\bibitem{CP}{\sc A. Cichocki, and A.H. Phan}, {\it Fast local algorithms for large scale nonnegative matrix and tensor factorizations},
           IEICE Trans. Fundamentals Electron. Commun. Comput. Sci., pp. 708--721, 2009.

\bibitem{CWY}{\sc Y.T. Chow, T. Wu, and W. Yin}, {\it Cyclic coordinate-update algorithms for fixed-point problems:
           Analysis and applications}, SIAM J. Sci. Comput., pp. A1280--A1300, 2017.

\bibitem{CZA}{\sc A. Cichocki, R. Zdunek, and S.I. Amari}, {\it Hierarchical ALS algorithms for nonnegative matrix and 3d tensor
           factorization}, in Independent Component Analysis and Signal Separation, Lecture Notes in Comput. Sci. 4666,
           Springer, New York, 2007, pp. 169--176.

\bibitem{CZPA}{\sc A. Cichocki, R. Zdunek, A.H. Phan, and S.I. Amari}, {\it Nonnegative matrix and tensor factorizations:
          Applications to exploratory multi-way data analysis and blind source separation}, Hoboken, NJ, USA: Wiley, 2009.

\bibitem{D}{\sc K. Devarajan}, {\it Nonnegative matrix factorization: An analytical and interpretive tool in computational biology},
           PLoS Comput. Biol. e1000029, 2008.

\bibitem{DDP}{\sc R. Du, B. Drake, and H. Park},
{\it Hybrid clustering based on content and connection structure using joint nonnegative matrix factor- ization}, J. Glob. Optim., pp. 1-17, 2017.

\bibitem{DKDP}{\sc R. Du, D. Kuang, B. Drake, and H. Park}, {\it DC-NMF: nonnegative matrix factorization based on divide-and-conquer
          for fast clustering and topic modeling}, J. Glob. Optim., pp. 777--798, 2017.

\bibitem{dkdp}{\sc R. Du, D. Kuang, B. Drake, and H. Park}, {\it Hierarchical community detection via-rank-2 symmetric nonnegative
          matrix factorization}, Comput. Soc. Netw., pp. 4--7, 2017.

\bibitem{DS}{\sc I. Dhillon, and S. Sra}, {\it Generalized nonnegative matrix approximations with bregman divergences},
Advances in Neural Inf. Proc. Systems 18, MIT Press, 2006, pp. 283--290.

\bibitem{EMWK}{\sc N.B. Erichson, A. Mendible, S. Wihlborn, and J.N. Kutz}, {\it Randomized nonnegative matrix factorization},
           Pattern Recognit. Lett., 2018, Doi:10.1016/j.patrec.2018.01.007.

\bibitem{G}{\sc N. Gillis}, {\it Introduction to nonnegative matrix factorization}, SIAG/OPT Views and News, pp. 7--16, 2017.

\bibitem{GKH}{\sc N. Gillis, D. Kuang, and H. Park},
{\it Hierarchical clustering of hyperspectral images using rank-two nonnegative matrix 
factorization}, 
IEEE Transactions on Geoscience and Remote Sensing, Vol. 53, No. 4, pp. 2066-2078, 2015 

\bibitem{H}{\sc P.O. Hoyer}, {\it Non-negative matrix factorization with sparseness constraints}, J. Mach. Learn. Res., pp. 1457--1469, 2004.

\bibitem{Ho}{\sc N.D. Ho}, {\it Nonnegative matrix factorization algorithms and applications}, Ph.D. thesis, Univ. Catholique de Louvain, 2008.


\bibitem{HY}{\sc Z. He, and X. Yuan}, {\it Block iteratively reweighted algorithms for robust symmetric nonnegative matrix factorization},
          IEEE Sign. Proc. Lett., pp. 1510--1514, 2018.


\bibitem{K}{\sc J. Kim}, {\it Nonnegative matrix and tensor factorizations, least squares problems, and applications}, Ph.D. Thesis,
         Georgia Institute of Technology, 2011.

\bibitem{KDP}{\sc D. Kuang, C. Ding, and H. Park}, {\it Symmetric nonnegative matrix factorization for graph clustering},
        in Proc. SIAM Int. Conf. Data Mining, 2012, pp. 106--117.

\bibitem{KDDP}{\sc D. Kuang, R. Du, B. Drake, and H. Park},
{\it DC-NMF: Nonnegative matrix factorization based on divide-and-conquer for fast clustering and topic modeling}, J. Glob. Optim., 68-4:777-798, 2017.

\bibitem{KHP}{\sc J. Kim, Y. He, and H. Park}, {\it Algorithms for nonnegative matrix and tensor factorizations: A unified view
         based on block coordinate descent framework}, J. Glob. Optim., pp. 285--319, 2014.

\bibitem{KP}{\sc J. Kim, and H. Park}, {\it Sparse non-negative matrix factorizations via alternating non-negativity-constrained
           least squares for microarray data analysis}, Bioinf., pp. 1495--1502, 2007.

\bibitem{KP1}{\sc J. Kim, and H. Park}, {\it Non-negative matrix factorization based on alternating non-negativity constrained
          least squares and active set method}, SIAM J. Matrix Aanl. Appl., pp. 713--730, 2008.

\bibitem{KP2}{\sc J. Kim, and H. Park}, {\it Toward faster nonnegative matrix factorization: A new algorithm and comparisons},
          in Proc. 8th IEEE Int. Conf. Data Mining, 2008, pp. 353--362.

\bibitem{kp}{\sc J. Kim, and H. Park}, {\it Fast nonnegative matrix factorization: An active-set-like method and comparisons},
         SIAM J. Sci. Comput., pp. 3261--3281, 2011.

\bibitem{KPh}{\sc D. Kuang, and H. Park}, {\it Fast rank-2 nonnegative matrix factorization for hierarchical document clustering},
        in Proc. 19th ACM SIGKDD Int. Conf. on knowledge Discovery and Data Mining, KDD 13, New York: ACM; 2013, pp. 739--747.

\bibitem{KSD}{\sc D. Kim, S. Sra, and I.S. Dhillon}, {\it Fast newton-type methods for the least squares nonnegative matrix
         approximation problem}, in Pro. 2007 SIAM Int. Conf. Data Mining, 2007.

\bibitem{KYP}{\sc D. Kuang, S. Yun, and H. Park}, {\it SymNMF: Nonnegative low-rank approximation of a similarity matrix
         for graph clustering}, J. Glob. Optim., pp. 1--30, 2013.

\bibitem{L}{\sc C. Lin}, {\it Projected gradient methods for nonnegative matrix factorization}, Neural Comput., pp. 2756--2779, 2007.

\bibitem{LH}{\sc C.L. Lawson, and R.J. Hanson}, {\it Solving least squares problems}, Prentice Hall, New Jersey, 1974.

\bibitem{LLP}{\sc L. Li, G. Lebanon, and H. Park}, {\it Fast bregman divergence nmf using taylor expansion and coordinate descent},
        in Proc. 18th ACM SIGKDD Int. Conf. Knowledge Discovery and Data Mining, 2012, pp. 307--315.

\bibitem{LPGF}{\sc P. Luo, J. Peng, Z. Guan, and J. Fan}, {\it Dual regularized multi-view non-negative matrix factorization
         for clustering}, Neurocomputing, pp. 1--11, 2018.

\bibitem{LS}{\sc D.D. Lee, and H.S. Seung}, {\it Learning the parts of objects by non-negative matrix factorization},
         Nature, pp. 788--791, 1999.

\bibitem{ls}{\sc D.D. Lee, and H.S. Seung}, {\it Algorithms for non-negative matrix factorization},
          in Advances in Neural Inf. Proc. Systems 13, MIT Press, 2001, pp. 556--562.

\bibitem{LWP}{\sc Z. Li, X. Wu, and H. Peng}, {\it Nonnegative matrix factorization on
           orthogonal subspace}, Pattern Recognit. Lett., pp. 905--911, 2010.

\bibitem{LZ}{\sc H. Liu, and Y. Zhou}, {\it Rank-two residue iteration method for nonnegative matrix factorization},
            Neurocomputing, pp. 3305--3312, 2011.

\bibitem{MZ}{\sc M. Merritt, and Y. Zhang}, {\it An interior-point gradient method for large-scale totally nonnegative
             least squares problems}, J. Optim. Theory and Appl., pp. 191--202, 2005.

\bibitem{NW}{\sc H.W. Ng, and S. Winkler}, {\it A Data-driven approach to cleaning large face datasets}, in Proc.
            IEEE Int. Conf. Image Processing (ICIP), Paris, France, 2014, pp. 27--30.

\bibitem{PCX}{\sc X. Peng, D. Chen, and D. Xu}, {\it Semi-supervised least squares nonnegative matrix factorization
           and graph-based extension}, Neurocomputing, pp. 98--111, 2018.

\bibitem{PPP}{\sc V.P. Pauca, J. Piper, and R.J. Plemmons}, {\it Nonnegative matrix factorization for spectral data analysis},
             Linear Algebra Appl., pp. 29--47, 2006.

\bibitem{PSBP}{\sc V.P. Pauca, F. Shahnaz, M.W. Berry, and R.J. Plemmons}, {\it Text mining using nonnegative matrix factorizations},
           in Proc. SIAM Int. Conf. Data Mining, 2004, pp. 452--456.

\bibitem{PT}{\sc P. Paatero, and U. Tapper}, {\it Positive matrix factorization: A non-negative factor model with optimal
             utilization of error estimates of data values}, Environmetrics, pp. 111--126, 1994.

\bibitem{Ret}{\sc R. Fujimoto, et al.}, {\it A dynamic data driven application system for vehicle tracking},
            Procedia Comput. Sci., pp. 1203--1215, 2014.

\bibitem{SBF}{\sc A. Sapienza, A. Bessi, and E. Ferrara}, {\it Non-negative tensor factorization for human behavioral
          pattern mining in online games}, Information 2018, doi:10.3390/info9030066.

\bibitem{SWSL}{\sc J. Sun, Z. Wang, F. Sun, and H. Li}, {\it Sparse dual graph-regularized NMF for image co-clustering},
         Neurocomputing, pp. 156--165, 2018.

\bibitem{TKCJ}{\sc A. Tosyali, J. Kim, J. Choi, and M.K. Jeong}, {\it Regularized asymmetric nonnegative matrix factorization
        for clustering in directed networks}, Pattern Recognit. Lett., pp. 750--757, 2019.

\bibitem{V}{\sc S.A. Vavasis}, {\it On the complexity of nonnegative matrix factorization}, SIAM J. Optim., pp. 1364--1377, 2009.

\bibitem{WSZ}{\sc C. Wang, X. Song, and J. Zhang}, {\it Graph regularized nonnegative matrix factorization with sample diversity
          for image representation}, Eng. Appl. Artif. Intel., pp. 32--39, 2018.

\bibitem{WWZCX}{\sc B. Wu, E. Wang, Z. Zhu, W. Chen, and P. Xiao}, {\it Manifold NMF with $L_{21}$ norm for clustering},
          Neurocomputing, pp. 78--88, 2018.

\bibitem{WZ}{\sc Y. Wang, and Y. Zhang}, {\it Nonnegative matrix factorization: A comprehensive review},
         IEEE Trans. Knowl. Data Eng., pp. 1336--1353, 2013.

\bibitem{XLG}{\sc W. Xu, X. Liu, and Y. Gong}, {\it Document clustering based on non-negative matrix factorization},
         in Proc. Int. ACM SIGIR Conf. Research and Development in Informaion Retrieval, 2003, pp. 267--273.

\bibitem{YB}{\sc F. Yanez, and F. Bach}, {\it Primal-dual algorithms for non-negative matrix factorization with
         the Kullback-Leibler divergence}, in IEEE Int. Conf. on Acoustics, Speech and Signal Processing (ICASSP), 2017, 16967286.

\bibitem{zc}{\sc R. Zdunek, and A. Cichocki}, {\it Non-negative matrix factorization with quasi-newton optimization},
         in Proc. 8th Int. Conf. Artificial Intelligence and Soft Computing, 2006, pp. 870--879.

\bibitem{ZC}{\sc R. Zdunek, and A. Cichocki}, {\it Fast nonnegative matrix factorization algorithms using projected gradient
          approaches for large-scale problems}, Comput. Intell. Neurosci, 2008, 939567.

\bibitem{ZH}{\sc F. Zhu, and P. Honeine}, {\it Online kernel nonnegative matrix factorization}, Signal Proc., pp. 143--153, 2017.

\end{thebibliography}

==> experiment_old.tex <==
\section{Numerical Experiments}\label{sec5}
\setcounter{equation}{0}

Because comprehensive comparisons with many existing numerical methods for NMF in \cite{KHP}
have demonstrated that HALS/RRI \cite{CP,CZA,CZPA,Ho} and ANLS-BPP \cite{KHP} are two of the most effective methods for NMF,
in all our experiments, we just compare our algorithm ARkNLS(k=3) with three algorithms: HALS, ANLS-BPP and RTRI.


\subsection{Data sets}

We have used $7$ real-world data sets for our comparison, and their information is shown in Algorithm \ref{tab}.
Among them, three text data sets TDT2, Reuters21578 and 20Newsgroups are in sparse format,
four image data sets ORL, Facescurb, YaleB and Caltech256 are in  dense format, see Table \ref{tab}.
Detailed description of the database are as follows:

\emph{ORL \footnote{https://github.com/fengbingchun/NN_Test} (Olivetti Research Laboratory)}:
It taken from AT$\&$T Laboratories Cambridge, contains 400 images of 40 peoples (each person with 10 images),
including the factors such as expressions, with or without glass and postures. The
images have normal, sleepy, sad and surprising expressions. The original size of images is $92\times 112$ pixels.

\emph{Facescurb}: This database contains 106863 photos of 530 celebrities, 265 whom are male, and 265 female.
It is provided by Hong-Wei Ng and Stefan Winkler \cite{NW}. The initial images that make up this dataset were obtained
by searching for names of celebrities using Google Image Search. Subsequently, they ran the Haarcascade-based face detector
from OpenCV 2.4.7 on the images to obtain a set of faces for each celebrity name, with the requirement that a face must be
at least $96\times 96$ pixels. In our experiment, we use photos from 256 male, and scale the images to $96\times 96$ pixels.


\emph{The Yale Face Database B (YaleB) \footnote{http://vision.ucsd.edu/~iskwak/ExtYaleDatabase/Yale%20Face%20Database.htm}}: It contains 5760 single light source
images of 10 subjects, each seen under 576 viewing conditions (9 different poses and 64 illumination conditions of each person).
The images have normal, sleepy, sad and surprising expressions. A subset of 38 persons with 64 images of per people,
 i.e., 2432 images are used, and we scale the images to $100\times 100$ pixels in our experiment.

\emph{TDT2}: It corpus (Nist Topic Detection and Tracking corpus) consists of data collected during the first half of 1998
and taken from 6 sources, including 2 newswires (APW, NYT), 2 radio programs (VOA, PRI) and 2 television programs (CNN, ABC).
There are 11201 on-topic documents which are classified into 96 semantic categories. In this subset, those documents appearing
in two or more categories are removed, leaving us with 9394 documents and 30 classes of documents in total.


\emph{Reuters}: It corpus contains 21578 documents in 135 categories. We provide here the ModApte version. Those documents
with multiple category labels are discarded. It left us with 8213 documents in 65 categories. After preprocessing, this
corpus contains 18933 distinct terms.

\emph{20Newsgroups}: It is a collection of original website reports, contains
18846 documents that are partitioned into 20 different newsgroups (topic), and the number
of documents in each newsgroup is different.

\emph{Caltech256 \footnote{http://www.vision.caltech.edu/Image_Datasets/Caltech256/}}: It is a set of 256 object categories containing a total of 30607 images. It is collected by choosing a set of object categories, downloading examples from Google Images and then manually screening out all images that did not fit category. we scale the images to $96\times 96$ pixels in our experiment.

 The datasets TDT2, Reuters and 20Newsgrounps are downloaded from \emph{http://www.cad.zju.edu.cn/home/dengcai/}.


\begin{table}[tb]%\scriptsize
\caption{Data sets}\label{tab}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Data set} &{\textbf{Size}} &{\textbf{sparsity}}\\
\hline
    ORL & 10304 $\times$ 400 &0.01\%\\
    Facescurb &22631 $\times$ 9216 &0.39\%\\
    YaleB  & 10000 $\times$ 2432 &2.70\%\\
    TDT2  & 36771 $\times$ 9394  &99.65\%\\
    Reuters & 18933 $\times$ 8293 &99.75\%\\
  20Newsgroups  & 26214 $\times$ 18846 &99.66\%\\
  Caltech256    & 30607 $\times$ 9216  &1.00\%\\
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Numerical Results}
%\setcounter{equation}{0}
In all experiments,  we compare  the computational time (in seconds) and residuals of our algorithm ARkNLS(k=3) with
three algorithms: HALS, ANLS-BPP and RTRI. Each experiment will be repeated for 10 times, and the numerical results,
i.e., the CPU time in seconds, the residuals, are the mean values from the 10 runs.
In our experiments, $r=\{60,90,120, 150, 180\}$, the initial matrices $U$ and $V$ are generated as follows:
\begin{itemize}
\item $V={\rm rand}(n,r)$;
\item $U={\rm rand}(m,r)$, and $U(:, j)=U(:,j)/\|U(:, j)\|_2$, ~$j=1, \cdots, r$,
\end{itemize}
and the algorithms stop at the same iterations 100. Here in each iteration of
ARkNLS(k=3), HALS, ANLS-BPP and RTRI, the entire blocks of $U$ and $V$ are updated.

\begin{rem}
\begin{itemize}
\item The singularity problem in HALS can also be overcome via Case i) in Subsection \ref{singularity} without
        ${\bf u}_2$ and ${\bf u}_3$.
\item Similar to ARkNLS(k=3), we can also elaborate ARkNLS with $k=2$ and then we have Algorithm
named ARkNLS(k=2) with a similar strategy for avoiding rank deficient problem in NMF iteration, as follows:

Assume $q=r/2$ is an integer. Let
\[   U= \left[ \begin{array}{ccc} U_1 & \cdots & U_q \end{array}\right], \qquad
                  V= \left[ \begin{array}{ccc} V_1 & \cdots & V_q \end{array}\right], \qquad
                   U_1, \cdots, U_q \in \mathbb{R}^{m\times 2}, \quad V_1, \cdots, V_q\in \mathbb{R}^{n\times 2}.
\]
Denote
\[ U_i=\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right],
   \quad V_i=\left[ \begin{array}{cc} {\bf v}_1 & {\bf v}_2 \end{array}\right].
\]
Then columns of $U_i$ and $V_i$ can be adjusted via Case i) and Case ii) in Subsection \ref{singularity} without
${\bf u}_3$, such that the adjusted $U_i$ is of full column rank and the value of
$U_iV_i^T={\bf u}_1{\bf v}_1^T+{\bf u}_2{\bf v}_2^T$ remains unchanged.
%
%
%\begin{itemize}
%\item [i)] First, if ${\bf u}_1^T {\bf u}_1=0$,  then ${\bf u}_{1}={\bf 0}$,  and so ${\bf u}_{1}{\bf v}^T_{1}=0$. Set
%$$ {\bf u}_{1}(2i-1)=1, \qquad {\bf v}_{1}={\bf 0},$$
%where the first column ${\bf u}_1$ of $U_i$ is the $(2i-1)$-th column of $U$. Obviously, ${\bf u}_1\not= 0$ and the value of
%${\bf u}_{1}{\bf v}^T_{1}+{\bf u}_{2}{\bf v}^T_{2}$ remains unchanged.
%
%\item[ii)] Next, if ${\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
%              \left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right])=0$,
%then ${\bf u}_{1}$ and ${\bf u}_{2}$ are linearly dependent. Note that
%the second column ${\bf u}_2$ of $U_i$ is the $(2i)$-th column of $U$,
%this implies
%\[ {\bf u}_{2}=\alpha{\bf u}_{1}=\frac{\|{\bf u}_2\|}{\|{\bf u}_1\|}{\bf u}_{1}, \qquad {\bf u}_{1}{\bf v}^T_{1}+{\bf u}_{2}{\bf v}^T_{2}
%={\bf u}_{1}({\bf v}^T_{1}+\alpha{\bf v}^T_{2})={\bf u}_{1}({\bf v}_{1}+\alpha{\bf v}_{2})^T. \]
%Set
%\[ {\bf v}_{1}={\bf v}_{1}+\alpha{\bf v}_{2},~~ {\bf v}_{2}={\bf 0},~~ {\rm and}~~{\bf u}_{2}={\bf 0}.
%\]
%Subsequently, we further adjust ${\bf u}_{2}$ to ensure ${\bf u}_{1}$ and ${\bf u}_{2}$ are linear independent:
%\begin{itemize}
%\item if ${\bf u}_{1}(2i-1)\neq0$, set ${\bf u}_{2}(2i)=1$;
%\item otherwise, ${\bf u}_{1}(2i-1)=0$, set ${\bf u}_{2}(2i-1)=1$.
%\end{itemize}
%Clearly, the adjusted ${\bf u}_{1}$ and ${\bf u}_{2}$ are linear independent and
%the value of
%${\bf u}_{1}{\bf v}^T_{1}+{\bf u}_{2}{\bf v}^T_{2}$ remains unchanged.
%\end{itemize}

\item We have compared ARkNLS(k=2) and ARkNLS(k=3), see Figures~\ref{FigN1},
we observed that they achieves almost same efficiency while ARkNLS(k=3) achieves slightly higher accuracy.
\begin{figure}[!t]
\centering
\includegraphics[height=3.5cm,width=5.78cm]{ORLk150R.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORLk1_150ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORLk2_150ttR.png}
\caption{Comparison of  ARkNLS(k=2) and  ARkNLS(k=3)}\label{FigN1}
\end{figure}
Note that intuitively ARkNLS(k=3) should perform better than ARkNLS(k=2) in general since
 ARkNLS(k=3) updates one more column than ARkNLS(k=2) per updating step. In addition,
the leading term of the flops in each iteration of  ARkNLS(k=2) and ARkNLS(k=3) is the same, that is,
$4mnr+4(m+n)r^2$. Hence, we only focus on ARkNLS(k=3) in this paper.
\end{itemize}
\end{rem}

\begin{rem}
In order to solve the singularity bug in RTRI, the cyclic strategy
of updating the columns ${\bf u}_{i}$ and ${\bf u}_{i+1}$ (and also ${\bf v}_{i}$ and ${\bf v}_{i+1}$)
 for $i=1, 2, \cdots$ in RTRI is given up in \cite{LZ}, instead, two indices $s$ and $t$ are selected so that
${\bf u}_s$ and ${\bf u}_{t}$ are the two columns of $U$ which mostly violate the optimality conditions in terms
of the reduced gradient of $\|A-UV^T\|_F$, and then ${\bf v}_s$ and ${\bf v}_{t}$ are updated, this results in
another  algorithm called RTMRI. We have compared RTRI and RTMRI, see Figures~\ref{FigN2}, here we set the
parameter $\rho=0.001$ in RTMRI as it is done in \cite{LZ}.
We observed that RTMRI has no obvious advantage compared with RTRI, so we only compare RTRI with HALS, ARkNLS(k=3) and
ANLS-BPP in this paper.
\begin{figure}[!t]
\centering
\includegraphics[height=3.5cm,width=5.78cm]{RTRIORL_90ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{RTRIReuters_90ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{RTRIReuters_150ttR.png}
\caption{Comparison of RTRI and  RTMRI}\label{FigN2}
\end{figure}


\end{rem}






Our numerical results are shown in Figures~\ref{Fig2}--\ref{Fig11}.
Among these figures,
\begin{itemize}
\item figures on the left side are the changes of residual with iterations;
\item figures in the middle and on the right side are the changes of residue with cup time.
\end{itemize}

\begin{figure}[!t]
\centering
\includegraphics[height=3.5cm,width=5.78cm]{ORL60R.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORL1_60ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORL2_60ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{ORL90R.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORL1_90ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORL2_90ttR.png} \\~\\
\includegraphics[height=3.5cm,width=5.78cm]{ORL120R.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORL1_120ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORL2_120ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{ORL150R.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORL1_150ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{ORL2_150ttR.png}\\~\\
\includegraphics[height=5.5cm,width=5.78cm]{ORL180R.png}
\includegraphics[height=5.5cm,width=5.78cm]{ORL1_180ttR.png}
\includegraphics[height=5.5cm,width=5.78cm]{ORL2_180ttR.png}
\caption{Results of ORL.
}\label{Fig2}
\end{figure}



\begin{figure}[!t]
\centering
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub60R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub1_60ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub2_60ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub90R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub1_90ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub2_90ttR.png}~\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub120R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub1_120ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub2_120ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub150R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub1_150ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub2_150ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub180R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub1_180ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Facescrub2_180ttR.png}
\caption{Results of Facescrub. }\label{Fig20}
\end{figure}



\begin{figure}[!t]
\centering
\includegraphics[height=3.5cm,width=5.78cm]{YaleB60R.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB1_60ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB2_60ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{YaleB90R.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB1_90ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB2_90ttR.png}~\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{YaleB120R.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB1_120ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB2_120ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{YaleB150R.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB1_150ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB2_150ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{YaleB180R.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB1_180ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{YaleB2_180ttR.png}
\caption{Results of YaleB.  }\label{Fig4}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[height=3.5cm,width=5.78cm]{TDT260R.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT21_60ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT22_60ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{TDT290R.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT21_90ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT22_90ttR.png}~\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{TDT2120R.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT21_120ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT22_120ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{TDT2150R.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT21_150ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT22_150ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{TDT2180R.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT21_180ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{TDT22_180ttR.png}
\caption{Results of TDT2.}\label{Fig6}
\end{figure}



\begin{figure}[!t]
\centering
\includegraphics[height=3.5cm,width=5.78cm]{Reuters60R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters1_60ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters2_60ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Reuters90R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters1_90ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters2_90ttR.png}~\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Reuters120R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters1_120ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters2_120ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Reuters150R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters1_150ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters2_150ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Reuters180R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters1_180ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Reuters2_180ttR.png}
\caption{Results of Reuters. }\label{Fig8}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[height=3.5cm,width=5.78cm]{News60R.png}
\includegraphics[height=3.5cm,width=5.78cm]{News1_60ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{News2_60ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{News90R.png}
\includegraphics[height=3.5cm,width=5.78cm]{News1_90ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{News2_90ttR.png}~\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{News120R.png}
\includegraphics[height=3.5cm,width=5.78cm]{News1_120ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{News2_120ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{News150R.png}
\includegraphics[height=3.5cm,width=5.78cm]{News1_150ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{News2_150ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{News180R.png}
\includegraphics[height=3.5cm,width=5.78cm]{News1_180ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{News2_180ttR.png}
\caption{Results of 20Newsgroups. }\label{Fig10}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[height=3.5cm,width=5.78cm]{Caltech25660R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2561_60ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2562_60ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Caltech25690R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2561_90ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2562_90ttR.png}~\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Caltech256120R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2561_120ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2562_120ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Caltech256150R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2561_150ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2562_150ttR.png}\\~\\
\includegraphics[height=3.5cm,width=5.78cm]{Caltech256180R.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2561_180ttR.png}
\includegraphics[height=3.5cm,width=5.78cm]{Caltech2562_180ttR.png}
\caption{Results of Caltech256. }\label{Fig11}
\end{figure}



Main observations from Figures~\ref{Fig2}--\ref{Fig11} include the following:
\begin{itemize}
\item All 4 algorithms ARkNLS(k=3), ANLS-BPP,  HALS and RTRI converge quickly for sparse datasets TDT2, Reuters and 20Newsgroups.
\item On the side of accuracy, ANLS-BPP achieves higher accuracy than the rest algorithms, followed by ARkNLS(k=3).
\item On the side of efficiency, ARkNLS(k=3) is faster than the rest algorithms, follows by HALS, and among these two algorithms
       ARkNLS(k=3) achieves higher accuracy.
%\item %In RTRI, $A-UV^T+{\bf u}_s{\bf v}_s^T+{\bf u}_t {\bf v}_t^T$ is computed when updating
      %${\bf v}_s$ and ${\bf v}_t$, ${\bf u}_s$ and ${\bf u}_t$. This is very time consuming for large dense datasets, for example,
      % Facescurb and Caltech256. Hence,
      % The implementation of RTRI can be significantly optimized.
\end{itemize}
In conclusion, our new algorithm ARkNLS(k=3) achieves a promising performance in the sense that it strikes a good balance
between accuracy and efficiency and hence it provides state-of-the-art performance in terms of computational accuracy and cpu time.

%Real world Experiments (Old)
%\subsection{Experiments on Real World Data}

% Raw data can be found here: https://docs.google.com/spreadsheets/d/1QubjHxNd5fbrrWRzq49R3iq3Rr3UjqUcHzZWxTEniHg/edit?usp=sharing
%\begin{table}[ht]
%\caption{Convergence results on real world data.}\label{tbl:rwres}
%\begin{center}
%\begin{tabular}{cccccccccc}
%\hline
%\multirow{2}{*}{Dataset} & \multirow{2}{*}{Rank}   & \multicolumn{4}{c}{Total time (s)} & \multicolumn{4}{c}{Final relative error} \\
%     &  & BPP   & ARk & HALS & RTRI & BPP & ARk & HALS & RTRI \\
%\hline
%\multirow{5}{*}{TDT2}         & 60   & 219.83    & 20.54   & 248.14   & 68.81    & 0.7785 & 0.7788 & 0.7789  & 0.8579  \\
%                              & 90   & 293.64    & 32.65   & 372.46   & 113.99   & 0.7475 & 0.7477 & 0.7487  & 0.8581  \\
%                              & 120  & 367.64    & 47.40   & 490.81   & 161.95   & 0.7248 & 0.7247 & 0.7255  & 0.8599  \\
%                              & 150  & 456.10    & 63.94   & 645.02   & 223.75   & 0.7061 & 0.7063 & 0.7070  & 0.8571  \\
%                              & 180  & 535.12    & 83.00   & 1,000.85 & 283.73   & 0.6905 & 0.6904 & 0.6908  & 0.8586  \\
%                              \hline
%\multirow{5}{*}{Reuters21578} & 60   & 143.87    & 7.35    & 158.13   & 19.29    & 0.6933 & 0.6944 & 0.6938  & 0.7907  \\
%                              & 90   & 197.51    & 13.90   & 261.68   & 32.64    & 0.6634 & 0.6642 & 0.6645  & 0.7945  \\
%                              & 120  & 248.91    & 20.22   & 366.19   & 52.69    & 0.6400 & 0.6418 & 0.6409  & 0.7951  \\
%                              & 150  & 307.07    & 26.56   & 457.07   & 81.13    & 0.6198 & 0.6218 & 0.6202  & 0.7931  \\
%                              & 180  & 361.18    & 34.94   & 550.36   & 116.68   & 0.6020 & 0.6042 & 0.6023  & 0.7877  \\
%                              \hline
%\multirow{5}{*}{20Newsgroups} & 60   & 248.42    & 27.34   & 259.11   & 90.00    & 0.5892 & 0.5913 & 0.5912  & 0.6407  \\
%                              & 90   & 344.32    & 40.33   & 385.54   & 144.10   & 0.5574 & 0.5587 & 0.5599  & 0.6376  \\
%                              & 120  & 434.93    & 56.88   & 513.57   & 213.59   & 0.5344 & 0.5353 & 0.5368  & 0.6373  \\
%                              & 150  & 543.73    & 73.57   & 655.94   & 276.37   & 0.5164 & 0.5178 & 0.5177  & 0.6345  \\
%                              & 180  & 688.35    & 96.36   & 821.58   & 346.21   & 0.5009 & 0.5028 & 0.5022  & 0.6390  \\
%                              \hline
%\multirow{5}{*}{ORL}          & 60   & 139.93    & 2.41    & 83.47    & 24.01    & 0.1380 & 0.1397 & 0.1406  & 0.1399  \\
%                              & 90   & 196.90    & 3.58    & 124.87   & 40.02    & 0.1229 & 0.1249 & 0.1253  & 0.1251  \\
%                              & 120  & 270.70    & 5.03    & 165.83   & 58.67    & 0.1119 & 0.1141 & 0.1138  & 0.1153  \\
%                              & 150  & 565.25    & 6.24    & 205.87   & 71.61    & 0.1027 & 0.1053 & 0.1044  & 0.1095  \\
%                              & 180  & 5,468.14  & 7.53    & 252.73   & 91.28    & 0.0942 & 0.0979 & 0.0955  & 0.1086  \\
%                              \hline
%\multirow{5}{*}{Facescrub}    & 60   & 738.43    & 26.61   & 719.99   & 1,111.09 & 0.1593 & 0.1619 & 0.1637  & 0.2606  \\
%                              & 90   & 1,007.70  & 32.53   & 928.80   & 1,625.88 & 0.1432 & 0.1468 & 0.1483  & 0.2606  \\
%                              & 120  & 1,349.59  & 37.20   & 1,153.96 & 2,171.35 & 0.1322 & 0.1359 & 0.1373  & 0.2606  \\
%                              & 150  & 16,091.57 & 45.65   & 1,358.70 & 2,715.31 & 0.1239 & 0.1281 & 0.1289  & 0.2535  \\
%                              & 180  & 27,438.08 & 57.19   & 1,540.83 & 3,322.89 & 0.1172 & 0.1217 & 0.1221  & 0.2535  \\
%                              \hline
%\multirow{5}{*}{Caltech256}   & 60   & 936.74    & 34.07   & 952.20   & 1,422.98 & 0.2059 & 0.2090 & 0.2090  & 0.3016  \\
%                              & 90   & 1,297.59  & 41.38   & 1,231.56 & 2,040.38 & 0.1903 & 0.1941 & 0.1938  & 0.3016  \\
%                              & 120  & 1,730.30  & 50.04   & 1,432.44 & 2,783.30 & 0.1797 & 0.1835 & 0.1833  & 0.3016  \\
%                              & 150  & 21,772.73 & 62.22   & 1,716.07 & 3,448.13 & 0.1712 & 0.1757 & 0.1753  & 0.3016  \\
%                              & 180  & 36,291.04 & 76.08   & 1,926.86 & 4,354.60 & 0.1645 & 0.1691 & 0.1685  & 0.3016  \\
%                              \hline
%\multirow{5}{*}{YaleB}        & 60   & 176.69    & 4.70    & 145.04   & 127.10   & 0.1662 & 0.1691 & 0.1697  & 0.1700  \\
%                              & 90   & 243.75    & 6.11    & 196.30   & 193.46   & 0.1450 & 0.1483 & 0.1507  & 0.1498  \\
%                              & 120  & 309.54    & 8.30    & 245.38   & 262.49   & 0.1297 & 0.1337 & 0.1361  & 0.1382  \\
%                              & 150  & 580.33    & 10.15   & 302.29   & 332.77   & 0.1182 & 0.1223 & 0.1257  & 0.1320  \\
%                              & 180  & 1,641.32  & 11.72   & 392.32   & 412.58   & 0.1087 & 0.1130 & 0.1168  & 0.1303  \\
%  \hline
%\end{tabular}
%\end{center}
%\end{table}

%We run the four algorithms on the real world data described in~\Cref{tbl:rwdata}. We test a suite of approximation ranks with $r$ varying from 60 to 180 in increments of 30. Once again, we impose the 100 iterations stopping criteria on the methods. The final results are displayed in~\cref{tbl:rwres}.

%We can observe that in terms of relative error BPP, ARk, and HALS perform about the same while BPP is slightly better than ARk and HALS. RTRI is the worst algorithm of the lot and performs particularly poorly on the sparse text data sets. The computational efficiency of ARk is clearly demonstrated in these experiments where ARk is shown to take only a fraction of the time taken by the other methods. In some instances ARk completes its entire quota of 100 iterations before BPP completes its first iteration. HALS and RTRI are the next fastest methods with BPP taking the longest time for the larger values of $r$. Sample convergence plots for the 20Newsgroup and ORL datasets is shown in~\cref{fig:rwcase}. The findings from the synthetic benchmarks carry over to the real world datasets. We can conclude that ARk strikes a good balance between accuracy and computational efficiency and discovers good approximations much faster than the the other methods compared in this work.

%\begin{figure}[tb]
%\begin{subfigure}{.48\textwidth}
%\centering\includegraphics[width=0.7\linewidth]{fig/inset-20Newsgroups-60.pdf}
%\caption{20Newsgroups with $r=60$}\label{fig:20ng}
%\end{subfigure}
%\begin{subfigure}{.48\textwidth}
%\centering\includegraphics[width=0.7\linewidth]{fig/inset-ORL-60.pdf}
%\caption{ORL with $r=60$}\label{fig:orl}
%\end{subfigure}
%\caption{Some typical convergence plots for real world world data. ARk is able to achieve good approximation error in a fraction of the time taken by the other methods.}
%\label{fig:rwcase}
%\end{figure}


==> rankdeficient_June22.tex <==

\subsection{Avoiding Rank Deficient Rank-k NLS in ARkNLS Iteration}\label{singularity}
%\smallskip

The low rank factor matrices $U$ and $V$ in NMF (\ref{nmf}) play important roles in applications.  For example, 
in the blind source separation, the matrix $A$ stands for the observation matrix, the matrix $U$ plays the role of mixing 
matrix and the matrix $V$ expresses source signals. In topic modeling \cite{KDDP}, where $A$ is a term-document matrix, 
the normalized columns of $U$ can be interpreted as topics, and the corresponding columns of $V$ provides the topic distribution 
for the documents. If the matrix $V$ has zero columns, this implies that some of source signals may be lost through the process. 
Hence this singularity problem must be overcome in applications. In addition, if any of the columns of these factor matrices are 
computed as zeros, then not only the interpretation of the result becomes difficult but also the computed reduced
rank becomes lower than the pre specified reduced rank $r$ which may make the approximation less accurate.
More importantly, ARkNLS iteration assumes that the matrix $U_i$ or $V_i$ that
plays the role of the coefficient matrix in each iteration of NLS has full column rank, and when this is not the case, the algorithm will breakdown.
This situation is well known especially in
HALS/RRI for NMF (\ref{nmf}) which is based on the \emph{rank-1}
residue iteration method
where a typical problem of NLS is
\begin{equation}
\min_{{\bf v}_i\in \mathbb{R}^{n\times 1},{\bf v}_i\geq{\bf 0}}\|{\bf u}_i{\bf v}_i^T-
(A-\Sigma_{l\neq i}{\bf u}_l{\bf v}_l^T)\|_F^2.
\end{equation}
The optimal solution vector ${\bf v}_i$ is given by
${\bf v}_i={ {[(A-\Sigma_{l\neq i}{\bf u}_l{\bf v}_l^T)^T {\bf u}_i]_{+}}\over { \|{\bf u}_i\|^2}}$ and thus
it  will be zero if $(A-\Sigma_{l\neq i}{\bf u}_l{\bf v}_l^T)^T {\bf u}_i\leq 0$
or ${\bf u}_i \in null (A-\Sigma_{l\neq i}{\bf u}_l{\bf v}_l^T)^T$ \cite{KHP},
and when this zero vector becomes the coefficient 'matrix' in a later step,
the iteration will break down.
When $k \geq 1$, due to an analogous rank deficiency of the coefficient matrix
$U_i$ or $V_i$, the results in Theorem \ref{thm3} cannot be applied to solve
the NLS problem (\ref{V}). When the NLS problem in the ARkNLS context involves
a rank deficient matrix, we will call it a {\em singularity} problem.


Fortunately, in the context of NMF, we can modify the involved NLS problem during rank-k NLS iteration, to avoid such a singularity problem.
This is achieved by
adjusting the columns of $U_i$ and $V_i$ such that the ``new" $U_i$ and $V_i$ satisfy that
$U_i$ is of full column rank and  the value of
\[ U_iV_i^T={\bf u}_1{\bf v}_1^T+{\bf u}_2{\bf v}_2^T+{\bf u}_3{\bf v}_3^T \]
remains unchanged.
This kind of adjustment is motivated by the monotonicity property of our algorithm ARkNLS with $k=3$:
denote the new
$U_i$ and $V_i$ by $\mathcal{U}_i$ and $\mathcal{V}_i$,
respectively, satisfying
$U_i V_i= \mathcal{U}_i\mathcal{V}_i$. Compute $\mathcal{V}_i^*$ by
\[ \mathcal{V}_i^* =\arg \min_{\mathcal{V}\in \mathbb{R}^{n\times 3},\mathcal{V}\geq{\bf 0}}
     \|\mathcal{U}_i\mathcal{V}^T-(A-\sum_{l\neq i}U_lV_l^T)\|_F^2.
\]
Then we have
\[ \|   \mathcal{U}_{i} (\mathcal{V}_i^*)^T-(A-\sum_{l\neq i}U_lV_l^T)\|_F
     \leq \| \mathcal{U}_i \mathcal{V}_i^T-(A-\sum_{l\neq i}U_lV_l^T)\|_F
     =  \| U_i V_i^T-(A-\sum_{l\neq i}U_lV_l^T)\|_F, \]
which preserves the monotonicity property of our algorithm ARkNLS with $k=3$.


Assume that we are concerned with the $i$th block $U_i = \left[ \begin{array}{ccc} {\bf u}_1 & {\bf u}_2 & {\bf u}_{3}\end{array}\right]$
and $V_i=\left[ \begin{array}{ccc} {\bf v}_1 & {\bf v}_2 & {\bf v}_{3}\end{array}\right].$
%    H=A^TU_i,  \qquad  M=U^TU_i. 
Remark \ref{rank-deficient} in the previous subsection listed the cases when $U_i$ is rank deficient.
%Also note that for solving (\ref{Vi}) via \eqref{t2}, only two matrix-matrix products
%$H=A^TU_i$ and $M=U^TU_i$ are needed, and all of ${\bf r}_{1}$, ${\bf r}_{2}$,
%${\bf r}_{3}$, $a$, $b$, $d_{12}$, $d_{13}$, and $d_{23}$ can be invoked via $H$ and $M$
%as shown in Theorem \ref{thm3}. Therefore, we will show how we can detect singularity in terms of matrices $H$ and $M$ 
%which will have to be computed anyway for other parts of the computation.
%
%\hp{I am not sure whether we want to introduce $H$ and $M$ in this section, and keep track of indexing regaring the entire 
%problem, i.e., regarindg $H$ and $M$. It makes expressions complicated.
%If we simply state the key information without showing all details of indexing regarding $H$ and $M$, it will be much easier 
%to follow. For example, the values like $d_{ij}$, etc. defined in Theorem 4.1 can be used here. Then we can simply say by computing matrices
%$H$ and $M$, we can obtain all the values we need for singularity problem, and for programming, we can take care of all these 
%indexing. What do you think?
%Also I feel Algorithm in the next page is difficult to follow due to detailed indexing.
%How about describing many of those in high level descriptions? At least we need a lot more
%comments in the algorithm so that it is easy to see what is going in major steps in high level}
%
In the following, we show how the factors $U_i$ and $V_i$ can be adjusted
when $U_i$ is rank deficient.
Here, we are adjusting the matrix $U_i$ checking the linear independence of its columns from left and right, and adjust $V_i$ as needed.
\begin{itemize}
\item [Step~i)] In the first step, if ${\bf u}_1 =0$, then we replace this ${\bf u}_1$ with a nonzero vector while keeping the value of
${\bf u}_{1}{\bf v}^T_{1}$ unchanged.
Assume ${\bf u}_1 = 0$, and so ${\bf u}_1{\bf v}_1^T=0$.
Then set $ {\bf u}_{1}(3i-2)=1, \ {\bf v}_{1}={\bf 0}$. Since
the first column ${\bf u}_1$ of $U_i$ is the $(3i-2)$th column of $U$,
${\bf u}_{1}({3i-2})$ is the $(3i-2)$th element of ${\bf u}_{1}$.
Now elements of ${\bf u}_1$ are all zeros except it has only one nonzero element
${\bf u}_{1}(3i-2)=1$. Obviously, ${\bf u}_1\not= 0$ now and the value of
${\bf u}_{1}{\bf v}^T_{1}+{\bf u}_{2}{\bf v}^T_{2}+{\bf u}_{3}{\bf v}^T_{3}$ remains unchanged.

%We can check whether ${\bf u}_1 = 0$ from the relationship ${\bf u}_1^T {\bf u}_1=M(3i-2, 1)=0$.
%Meanwhile, the elements of $H$ and $M$ should also be adjusted:
%\[ H(:,1)=A(3i-2,:)^T,~~~M(:, 1)=U(3i-2,:)^T, ~~~M(3i-2, :)=U_i(3i-2, :).  \]

\item[Step~ii)] Now we have ${\bf u}_1\not= 0$.
But if ${\bf u}_1$ and ${\bf u}_2$ are linearly dependent, then we have
\[ {\bf u}_{2}=\alpha{\bf u}_{1}, \qquad {\bf u}_{1}{\bf v}^T_{1}+{\bf u}_{2}{\bf v}^T_{2}
={\bf u}_{1}({\bf v}^T_{1}+\alpha{\bf v}^T_{2})={\bf u}_{1}({\bf v}_{1}+\alpha{\bf v}_{2})^T, \]
where $\alpha=\frac{\|{\bf u}_2\|}{\|{\bf u}_1\|}$.
%We can check the linear dependence of ${\bf u}_1$ and ${\bf u}_2$ from the relationship
%\[ {\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
%              \left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right])={\rm det}(M(3i-2:3i-1, 1:2))=0. \]
%and
%\begin{align}\label{90}
%\alpha=\frac{\|{\bf u}_2\|}{\|{\bf u}_1\|} =\sqrt{\frac{M(3i-1,2)}{M(3i-2,1)}},
%\end{align}
We set
\begin{align}\label{f90}
{\bf v}_{1}={\bf v}_{1}+\alpha{\bf v}_{2},~~ {\bf v}_{2}={\bf 0},~~ {\rm and}~~{\bf u}_{2}={\bf 0}.
\end{align}
Note that the second column ${\bf u}_2$ of $U_i$ is the $(3i-1)$th column of $U$,
we further adjust ${\bf u}_{2}$ to ensure ${\bf u}_{1}$ and ${\bf u}_{2}$ are linearly independent:
\begin{equation} \label{case2-1}
 {\rm if \ }  {\bf u}_{1}(3i-2)\neq 0, {\rm \ set \ }
 {\bf u}_{2}(3i-1)=1; %~H(:,2)=A(3i-1,:)^T, ~M(:, 2)=U(3i-1,:)^T, ~M(3i-1,:)=U_i(3i-1, :); 
\end{equation}
\begin{equation}\label{case2-2} 
{\rm otherwise, \ set \ }  {\bf u}_{2}(3i-2)=1. 
\end{equation}
% ~H(:,2)=A(3i-2,:)^T, ~M(:, 2)=U(3i-2,:)^T, ~M(3i-1,:)=U_i(3i-2, :). \]
Clearly, the adjusted ${\bf u}_{1}$ and ${\bf u}_{2}$ are linearly independent and
${\bf u}_{1}{\bf v}^T_{1}+{\bf u}_{2}{\bf v}^T_{2}$ remains unchanged,
and therefore
${\bf u}_{1}{\bf v}^T_{1}+{\bf u}_{2}{\bf v}^T_{2}+{\bf u}_{3}{\bf v}^T_{3}$ remains unchanged.


\item[Step~iii)] Now ${\bf u}_1 $ and ${\bf u}_2$ are linearly independent.
Finally, if ${\bf u}_1$, ${\bf u}_2$ and  ${\bf u}_3$ are linearly dependent, i.e, \\
if
$\label{rank-con1}  {\rm rank}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right])
   ={\rm rank}(\left[ \begin{array}{ccc} {\bf u}_1 & {\bf u}_2 & {\bf u}_3 \end{array}\right])=2$,
then we have
\[ {\bf u}_{3}=\widetilde{\alpha}{\bf u}_{1}+\widetilde{\beta}{\bf u}_{2}, \]
%Note that we can check the condition (\ref{rank-con1}) from the relationship
%\[ {\rm det}(\left[ \begin{array}{ccc} {\bf u}_1 & {\bf u}_2 & {\bf u}_3 \end{array}\right]^T
%              \left[ \begin{array}{ccc} {\bf u}_1 & {\bf u}_2 & {\bf u}_3 \end{array}\right])=
%      {\rm det}(M(3i-2:3i,1:3))=0,  \]
%and furthermore,
where
\begin{eqnarray}\label{z1}
\widetilde{\alpha}=\frac{{\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
                                    \left[ \begin{array}{cc} {\bf u}_3 & {\bf u}_2 \end{array}\right])}
                        {{\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
                                    \left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]) }
%=\frac{M(3i-1,2)M(3i-2,3)-M(3i-1,3)M(3i-2,2)}{M(3i-1,2)M(3i-2,1)-(M(3i-1,1))^2},
\end{eqnarray}
and
\begin{eqnarray}\label{z2}
\widetilde{\beta}=\frac{{\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
                                    \left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_3 \end{array}\right])}
                        {{\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
                                    \left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]) }.
%=\frac{M(3i-2,1)M(3i-1,3)-M(3i-2,2)M(3i-2,3)}{M(3i-1,2)M(3i-2,1)-(M(3i-1,1))^2}.
\end{eqnarray}
Actually, $\widetilde{\alpha}$ and $\widetilde{\beta}$ cannot be both negative as ${\bf u}_1$, ${\bf u}_2$ and ${\bf u}_{3}$ are all
nonnegative, ${\bf u}_1\not=0$ and ${\bf u}_2\not=0$. But it is possible that $\widetilde{\alpha}<0$ or $\widetilde{\beta}<0$.
If this happens, we need to permute the index set $\left[ \begin{array}{ccc} 1 & 2 & 3 \end{array}\right]$ to the set
$\mathcal{I}=\left[ \begin{array}{ccc} \mathcal{I}(1) & \mathcal{I}(2) & \mathcal{I}(3) \end{array}\right]$
and change the values of $\widetilde{\alpha}$ and $\widetilde{\beta}$ such that
\[ {\bf u}_{\mathcal{I}(3)}=\widetilde{\alpha} {\bf u}_{\mathcal{I}(1)}+\widetilde{\beta} {\bf u}_{\mathcal{I}(2)},
   \quad \widetilde{\alpha}\geq 0, \quad \widetilde{\beta}\geq 0. \]
In such a way, ${\bf u}_{\mathcal{I}(1)}$ and ${\bf u}_{\mathcal{I}(2)}$ must be linearly independent. So we
can adjust ${\bf v}_1$, ${\bf v}_2$ and ${\bf v}_3$ easily and meanwhile we only need to
adjust ${\bf u}_{\mathcal{I}(3)}$ such that the adjusted ${\bf u}_1$, ${\bf u}_2$ and ${\bf u}_3$ are linearly independent,
and the value of $U_iV_i^T={\bf u}_1{\bf v}_1+{\bf u}_2{\bf v}_2+{\bf u}_3{\bf v}_3$ remains unchanged.
The permuted index set $\mathcal{I}=\left[ \begin{array}{ccc} \mathcal{I}(1) & \mathcal{I}(2) & \mathcal{I}(3) \end{array}\right]$
can be obtained as follows:
\begin{itemize}
\item if $\widetilde{\alpha}\widetilde{\beta}\geq 0$,
then $\widetilde{\alpha}\geq 0$, $\widetilde{\beta}\geq 0$, and
${\bf u}_{3}=\widetilde{\alpha}{\bf u}_{1}+\widetilde{\beta}{\bf u}_{2}$. Let
\[ \mathcal{I}=\left[ \begin{array}{ccc} 1 & 2 & 3\end{array}\right], \quad
   \mathcal{J}=\left[ \begin{array}{ccc} 3i-2 & 3i-1 & 3i \end{array}\right]; \]
\item if $\widetilde{\alpha}<0$, $\widetilde{\beta}>0$, then ${\bf u}_{2}
          =-\frac{\widetilde{\alpha}}{\widetilde{\beta}}{\bf u}_{1}+\frac{1}{\widetilde{\beta}}{\bf u}_{3}$
with $-\frac{\widetilde{\alpha}}{\widetilde{\beta}}>0$ and $\frac{1}{\widetilde{\beta}}>0$.
Let
\[ \widetilde{\alpha}={-\widetilde{\alpha}}/{\widetilde{\beta}}>0,
    ~~~\widetilde{\beta}={1}/{\widetilde{\beta}}>0,~~~
    \mathcal{I}=\left[ \begin{array}{ccc} 1 & 3 & 2\end{array}\right], \quad
    \mathcal{J}=\left[ \begin{array}{ccc} 3i-2 & 3i & 3i-1\end{array}\right]; \]
\item if $\widetilde{\alpha}>0$, $\widetilde{\beta}<0$, then
       ${\bf u}_{1}=-\frac{\widetilde{\beta}}{\widetilde{\alpha}}{\bf u}_{2}+\frac{1}{\widetilde{\alpha}}{\bf u}_{3}$
       with $-\frac{\widetilde{\beta}}{\widetilde{\alpha}}>0$ and $\frac{1}{\widetilde{\alpha}}>0$.
Let
\[ \widetilde{\alpha}=-{\widetilde{\beta}}/{\widetilde{\alpha}}>0,~~~
     \widetilde{\beta}={1}/{\widetilde{\alpha}}>0,~~~
     \mathcal{I}=\left[ \begin{array}{ccc} 2 & 3 & 1\end{array}\right], \quad
     \mathcal{J}=\left[ \begin{array}{ccc} 3i-1 & 3i & 3i-2\end{array}\right].\]
\end{itemize}
Now we have
\[ {\bf u}_{\mathcal{I}(3)}=\widetilde{\alpha} {\bf u}_{\mathcal{I}(1)}+\widetilde{\beta} {\bf u}_{\mathcal{I}(2)},
   \quad \widetilde{\alpha}\geq 0, \ \widetilde{\beta}\geq 0, \]
and ${\bf u}_{\mathcal{I}(j)}$ is the $\mathcal{J}(j)$-th column of $U$, $j=1, 2, 3$.
Moreover, we also have
\begin{eqnarray*}
 {\bf u}_1{\bf v}_1^T+ {\bf u}_2{\bf v}_2^T+ {\bf u}_3{\bf v}_3^T
  &=& {\bf u}_{\mathcal{I}(1)} {\bf v}^T_{\mathcal{I}(1)}+
   {\bf u}_{\mathcal{I}(2)}{\bf v}^T_{\mathcal{I}(2)} +
   {\bf u}_{\mathcal{I}(3)} {\bf v}^T_{\mathcal{I}(3)}  \\
   &=& {\bf u}_{\mathcal{I}(1)}( {\bf v}_{\mathcal{I}(1)} + \widetilde{\alpha} {\bf v}_{\mathcal{I}(3)})^T
   +{\bf u}_{\mathcal{I}(2)}( {\bf v}_{\mathcal{I}(2)} + \widetilde{\beta} {\bf v}_{\mathcal{I}(3)})^T.
\end{eqnarray*}
Thus, we set
\[ {\bf v}_{\mathcal{I}(1)}={\bf v}_{\mathcal{I}(1)}+\widetilde{\alpha}{\bf v}_{\mathcal{I}(3)},~~~
           {\bf v}_{\mathcal{I}(2)}={\bf v}_{\mathcal{I}(2)}+\widetilde{\beta}{\bf v}_{\mathcal{I}(3)},
           ~~~{\bf v}_{\mathcal{I}(3)}={\bf 0},~~~{\bf u}_{\mathcal{I}(3)}={\bf 0}.  \]
then ${\bf v}_{\mathcal{I}(1)}$ and ${\bf v}_{\mathcal{I}(2)}$ are both nonnegative vectors,
${\bf u}_{\mathcal{I}(1)}$ and ${\bf u}_{\mathcal{I}(2)}$ are linearly independent, and the value of
${\bf u}_{1}{\bf v}^T_{1}+{\bf u}_{2}{\bf v}^T_{2}+{\bf u}_{3}{\bf v}^T_{3}$ remains unchanged.

Now we adjust ${\bf u}_{\mathcal{I}(3)}$ so that ${\bf u}_{1},{\bf u}_{2}$, ${\bf u}_{3}$ are linearly independent
and the value of ${\bf u}_{1}{\bf v}^T_{1}+{\bf u}_{2}{\bf v}^T_{2}+{\bf u}_{3}{\bf v}^T_{3}$ remains unchanged:
\begin{equation}\label{case3-1}
 {\rm if \ } {\bf u}_{\mathcal{I}(1)}(\mathcal{J}(1)){\bf u}_{\mathcal{I}(2)}(\mathcal{J}(2))
     -{\bf u}_{\mathcal{I}(1)}(\mathcal{J}(2)){\bf u}_{\mathcal{I}(2)}(\mathcal{J}(1))\neq 0, 
     {\rm \ set \ }
         {\bf u}_{\mathcal{I}(3)}(\mathcal{J}(3))=1;  
\end{equation}
% \quad H(:,\mathcal{I}(3))=A(\mathcal{J}(3),:)^T,\quad
%             M(:,\mathcal{I}(3))=U(\mathcal{J}(3),:)^T,
%        \quad M(\mathcal{J}(3),:)=U_i(\mathcal{J}(3), :); \]
\begin{equation}\label{case3-2}
{\rm  Otherwise,\  if \ } {\bf u}_{\mathcal{I}(1)}(\mathcal{J}(1))+{\bf u}_{\mathcal{I}(2)}(\mathcal{J}(1))=0,
 {\rm \ set \ }
     {\bf u}_{\mathcal{I}(3)}(\mathcal{J}(1))=1; 
\end{equation}
%\quad H(:,\mathcal{I}(3))=A(\mathcal{J}(1),:)^T,\quad
%                M(:,\mathcal{I}(3))=U(\mathcal{J}(1),:)^T, \quad
%                M(\mathcal{J}(3),:)=U_i(\mathcal{J}(1), :);\]
\begin{equation}\label{case3-3}
{\rm else \ if \ }  {\bf u}_{\mathcal{I}(1)}(\mathcal{J}(1))+{\bf u}_{\mathcal{I}(2)}(\mathcal{J}(1))\neq 0,
   {\rm \ set \ }
 {\bf u}_{\mathcal{I}(3)}(\mathcal{J}(2))=1. 
\end{equation}
% \quad H(:,\mathcal{I}(3))=A(\mathcal{J}(2),:)^T, \quad
%   M(:,\mathcal{I}(3))=U(\mathcal{J}(2),:)^T, \quad
%    M(\mathcal{J}(3),:)=U_i(\mathcal{J}(2), :). \]
\end{itemize}


Through the above three steps, $U_i$ is of full column rank and so Theorem \ref{thm3} can be applied.


\subsection{Algorithm ARkNLS with $k=3$}
\se{I think we need $M=U^TU$ instead of $U^T U_i$ for correctness when updating the inner products once $\bf u_1$ changes (please verify)}
Denote
\[    H=A^TU_i,  \qquad  M=U^TU. \]
Note that for solving (\ref{Vi}) via \eqref{t2}, only two matrix-matrix products $H$ and $M$ are needed, and 
all of ${\bf r}_{1}$, ${\bf r}_{2}$, ${\bf r}_{3}$, $a$, $b$, $d_{12}$, $d_{13}$, and $d_{23}$ can be invoked via $H$ and $M$
as shown in Theorem \ref{thm3}. Moreover, the singularity problem discussed in the subsection above can be detected via
matrices $H$ and $M$ which will have to be computed anyway for other parts of the computation.

In the following we illustrate the implementation of adjustment of vectors ${\bf u}_1$, ${\bf u}_2$ and ${\bf u}_3$
first and then present Algorithm ARkNLS(k=3).

\begin{itemize}
\item In Step i), whether ${\bf u}_1 = 0$ can be checked from the relationship ${\bf u}_1^T {\bf u}_1=M(3i-2,3i-2)=0$.
After ${\bf u}_1$ is adjusted, the elements of $H$ and $M$ should also be adjusted:
\[ H(:,1)=A(3i-2,:)^T,~~~M(:, 1)=U(3i-2,:)^T, ~~~M(3i-2, :)=U(3i-2, :).  \]

\item In Step ii), the linear dependence of ${\bf u}_1$ and ${\bf u}_2$ can be checked from the relationship
\[ {\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
              \left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right])={\rm det}(M(3i-2:3i-1,3i-2:3i-1))=0, \]
and moreover,
\[ \alpha=\frac{\|{\bf u}_2\|}{\|{\bf u}_1\|} =\sqrt{\frac{M(3i-1,3i-1)}{M(3i-2,3i-2)}}.
\]
Furthermore, After ${\bf u}_2$ is adjusted, the elements of $H$ and $M$ should also be adjusted:
\begin{itemize}
\item Corresponding to (\ref{case2-1}),
\[ H(:,2)=A(3i-1,:)^T, ~M(:, 2)=U(3i-1,:)^T, ~M(3i-1,:)=U(3i-1, :); \]
\item Corresponding to (\ref{case2-2}),
\[ H(:,2)=A(3i-2,:)^T, ~M(:, 2)=U(3i-2,:)^T, ~M(3i-1,:)=U(3i-2, :). \]
\end{itemize}

\item In Step iii), the condition (\ref{rank-con1}) can be checked from the relationship
\[ {\rm det}(\left[ \begin{array}{ccc} {\bf u}_1 & {\bf u}_2 & {\bf u}_3 \end{array}\right]^T
              \left[ \begin{array}{ccc} {\bf u}_1 & {\bf u}_2 & {\bf u}_3 \end{array}\right])=
      {\rm det}(M(3i-2:3i,3i-2:3i))=0.  \]
In addition,
\[
\widetilde{\alpha}=\frac{{\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
                                    \left[ \begin{array}{cc} {\bf u}_3 & {\bf u}_2 \end{array}\right])}
                        {{\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
                                    \left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]) }
=\frac{M(3i-1,3i-1)M(3i-2,3i)-M(3i-1,3i)M(3i-2,3i-1)}{M(3i-1,3i-1)M(3i-2,3i-2)-(M(3i-1,3i-2))^2},
\]
and
\[
\widetilde{\beta}=\frac{{\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
                                    \left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_3 \end{array}\right])}
                        {{\rm det}(\left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]^T
                                    \left[ \begin{array}{cc} {\bf u}_1 & {\bf u}_2 \end{array}\right]) }
=\frac{M(3i-2,3i-2)M(3i-1,3i)-M(3i-2,3i-1)M(3i-2,3i)}{M(3i-1,3i-1)M(3i-2,3i-2)-(M(3i-1,3i-2))^2}.
\]
After ${\bf u}_{\mathcal{I}(3)}$ is adjusted, the elements of $H$ and $M$ should also be adjusted:
\begin{itemize}
\item Corresponding to (\ref{case3-1}),
\[     H(:,\mathcal{I}(3))=A(\mathcal{J}(3),:)^T,\quad
       M(:,\mathcal{I}(3))=U(\mathcal{J}(3),:)^T, \quad 
       M(\mathcal{J}(3),:)=U(\mathcal{J}(3), :); \]

\item Corresponding to (\ref{case3-2}),
\[      H(:,\mathcal{I}(3))=A(\mathcal{J}(1),:)^T,\quad
        M(:,\mathcal{I}(3))=U(\mathcal{J}(1),:)^T, \quad
        M(\mathcal{J}(3),:)=U(\mathcal{J}(1), :);   \]

\item Corresponding to  (\ref{case3-3}),
\[      H(:,\mathcal{I}(3))=A(\mathcal{J}(2),:)^T, \quad
        M(:,\mathcal{I}(3))=U(\mathcal{J}(2),:)^T, \quad
        M(\mathcal{J}(3),:)=U(\mathcal{J}(2), :). \]
\end{itemize}

\end{itemize}


Theorem \ref{thm3} and discussions above lead to Algorithm-ARkNLS(k=3) for NMF problem.


\begin{algorithm}%[H]
\caption{Alternating \emph{Rank-3 NLS} for NMF (ARkNLS(k=3))} \label{alg2}
\begin{algorithmic}
\STATE 1.~Given a $m$-by-$n$ nonnegative matrix $A$. Initialize $U\in \mathbb{R}^{m\times r}$, $V\in \mathbb{R}^{n\times r}$
with nonnegative elements and normalized the columns of $U$. Let $q={\tt floor}(\frac{r}{3})$, where ${\tt floor}(\frac{r}{3})$
rounds $\frac{r}{3}$ to the nearest integer less than or equal to $\frac{r}{3}$
\STATE 2.~\textbf{Repeat} 
\STATE 3.~\textbf{For} $i=1:q$ \textbf{do} \qquad \qquad\quad
                       \  \% $U_i=\left[ \begin{array}{ccc} {\bf u}_1 & {\bf u}_2 & {\bf u}_3 \end{array}\right]$,
                         ${\bf u}_1=U(:, 3i-2), ~{\bf u}_2=U(:, 3i-1), ~{\bf u}_3=U(:, 3i)$.
%\STATE 4.~Let $H=A^TU_i$, $M=U^TU_i$. 
%\ \% For the implementation of (\ref{Vi}) 
%with \eqref{t2}, it only needs to compute
%\STATE    \hskip 5cm  \% the two matrix-matrix %products $H=A^TU_i$ and $M=U^TU_i$,
%\STATE    \hskip 5cm  \% then all of $r_{1}$, $r_{2}$, $r_{3}$, $a$, $b$, $d_{12}$, $d_{13}$, and $d_{23}$ can be invoked via $H$ and $M$.

\STATE 4. Adjust the columns of $U_i$ and $V_i$ such that the adjusted $U_i$ is of full column rank and the value of $U_iV_i^T$
\STATE \qquad remains unchanged. 
%Meanwhile, the elements of $H$ and $M$ are 
%also adjusted accordingly.
%               
%               
%               
%\STATE 5.~~~~\textbf{if}~~$M(3i-2,1)=0$, \textbf{then}
%                         \% $V_i=\left[ \begin{array}{ccc} {\bf v}_1 & {\bf v}_2 & {\bf v}_3 \end{array}\right]$,
%                         ${\bf v}_1=V(:, 3i-2), ~{\bf v}_2=V(:, 3i-1), ~{\bf v}_3=V(:, 3i)$.
%\STATE 6.~~~~~~~${\bf v}_{1}={\bf 0}$,~~${\bf u}_{1}(3i-2)=1$,~~$H(:,1)=A(3i-2,:)^T$,
%\STATE 7.~~~~~~~$M(:, 1)=U(3i-2,:)^T,~M(3i-2,:)=U_i(3i-2, :)$;
%\STATE 8.~~~~\textbf{end if}
%\STATE 9.~~~~\textbf{if}~~$M(3i-2,1)M(3i-1,2)-(M(3i-2,2))^2=0$, \textbf{then}
%\STATE 10.~~~~~${\bf v}_{1}={\bf v}_{1}+\sqrt{\frac{M(3i-1,2)}{M(3i-2,1)}}{\bf v}_{2}$,
%        ~~${\bf v}_{2}={\bf 0}$,~~${\bf u}_{2}={\bf 0}$,
%\STATE 11.~~~~~\textbf{if} ${\bf u}_{1}(3i-2)\neq0$, \textbf{then}
%\STATE 12.~~~~~~~{\small${\bf u}_{2}(3i-1)=1$,~$H(:,2)=A(3i-1,:)^T$,~$M(:, 2)=U(3i-1,:)^T$,~$M(3i-1,:)=U_i(3i-1, :)$.}
%\STATE 13.~~~~~\textbf{else}
%\STATE 14.~~~~~~~{\small${\bf u}_{2}(3i-2)=1$,~$H(:,2)=A(3i-2,:)^T$,~$M(:, 2)=U(3i-2,:)^T$, ~$M(3i-1,:)=U_i(3i-2,:)$. }
%\STATE 15.~~~\textbf{end if}
%\STATE 16.~~~\textbf{if}~~${\rm det}(M(3i-2:3i,1:3)=0$, \textbf{then}
%\STATE 17.~~~~~Compute $\widetilde{\alpha}$ via \eqref{z1}, $\widetilde{\beta}$ via \eqref{z2},
%let $\mathcal{I}=\left[ \begin{array}{ccc} 1 & 2 & 3\end{array}\right]$
% %                     and $\mathcal{J}=\left[ \begin{array}{ccc} 3i-2 & 3i-1 & 3i\end{array}\right]$.
%\STATE 18.~~~~~\textbf{if}~~$\widetilde{\alpha}<0$,
%\STATE 19.~~~~~ \textbf{then} \quad $\widetilde{\alpha}={-\widetilde{\alpha}}/{\widetilde{\beta}}$,\quad
%$\widetilde{\beta}={1}/{\widetilde{\beta}}$,\quad  $\mathcal{I}=\left[ \begin{array}{ccc} 1 & 3 & 2\end{array}\right]$
%            and $\mathcal{J}=\left[ \begin{array}{ccc} 3i-2 & 3i & 3i-1\end{array}\right]$, ~~~\textbf{end if}.
%\STATE 20.~~~~~\textbf{if}~~$\widetilde{\beta}<0$,
%\STATE 21.~~~~~\textbf{then} \quad $\widetilde{\alpha}=-{\widetilde{\beta}}/{\widetilde{\alpha}}$, \quad
%$\widetilde{\beta}={1}/{\widetilde{\alpha}}$, \quad $\mathcal{I}=\left[ \begin{array}{ccc} 2 & 3 & 1\end{array}\right]$
%            and $\mathcal{J}=\left[ \begin{array}{ccc} 3i-1 & 3i & 3i-2\end{array}\right]$, ~~~\textbf{end if}.
%\STATE 22.~~~~~${\bf v}_{\mathcal{I}(1)}={\bf v}_{\mathcal{I}(1)}+\widetilde{\alpha}{\bf v}_{\mathcal{I}(3)}$,\quad
%${\bf v}_{\mathcal{I}(2)}={\bf v}_{\mathcal{I}(2)}+\widetilde{\beta}{\bf v}_{\mathcal{I}(3)}$,\quad
%       ${\bf v}_{\mathcal{I}(3)}={\bf 0}$, \quad ${\bf u}_{\mathcal{I}(3)}={\bf 0}$.
%\STATE 23.~~~~~\textbf{if} ${\bf u}_{\mathcal{I}(1)}(\mathcal{J}(1)){\bf u}_{\mathcal{I}(2)}(\mathcal{J}(2))
%     -{\bf u}_{\mathcal{I}(1)}(\mathcal{J}(2)){\bf u}_{\mathcal{I}(2)}(\mathcal{J}(1))\neq0$,
%\STATE 24.~~~~~~~~${\bf u}_{\mathcal{I}(3)}(\mathcal{J}(3))=1$,~$H(:,\mathcal{I}(3))=A(\mathcal{J}(3),:)^T$,
%     ~$M(:, \mathcal{I}(3))=U(\mathcal{J}(3),:)^T$, ~$M(\mathcal{J}(3), :)=U_i(\mathcal{J}(3), :)$.
%\STATE 25.~~~~~\textbf{else}
%\STATE 26.~~~~~~~~\textbf{if} ${\bf u}_{\mathcal{I}(1)}(\mathcal{J}(1))+{\bf u}_{\mathcal{I}(2)}(\mathcal{J}(1))=0$, \textbf{then}
%\STATE 27.~~~~~~~~~~~${\bf u}_{\mathcal{I}(3)}(\mathcal{J}(1))=1$,~$H(:,\mathcal{I}(3))=A(\mathcal{J}(1),:)^T$,
%       ~$M(:, \mathcal{I}(3))=U(\mathcal{J}(1),:)^T$, ~$M(\mathcal{J}(3), :)=U_i(\mathcal{J}(1), :)$.
%\STATE 28.~~~~~~~~\textbf{else}
%\STATE 29.~~~~~~~~~~~${\bf u}_{\mathcal{I}(3)}(\mathcal{J}(2))=1$,~~$H(:,\mathcal{I}(3))=A(\mathcal{J}(2),:)^T$,
%         ~$M(:, \mathcal{I}(3))=U(\mathcal{J}(2),:)^T$, ~~$M(\mathcal{J}(3), :)=U_i(\mathcal{J}(2), :)$.
%\STATE 30.~~~~~\textbf{end if}
%\STATE 31.~~~\textbf{end if}
\STATE 5.~Compute $V_i$ by (\ref{Vi}) with  \eqref{t2}.
\STATE 6.~\textbf{End for}

\STATE 7.~\textbf{If} ${\tt mod}(r,3)=1 {\rm ~or~} 2$ \textbf{then} compute ${{\bf v}}_{r-2}$, ${{\bf v}}_{r-1}$, ${{\bf v}}_{r}$
               via the above Steps 4--5. \textbf{End if}
\STATE       \hskip 5cm \% ${\tt mod}(r,3)$ returns the remainder after division of $r$ by $3$.
\STATE
\STATE       \hskip 5cm \% In the case ${\tt mod}(r,3)=1$, ${\bf u}_{r-2}$ and ${\bf u}_{r-1}$ must be linearly independent 
\STATE       \hskip 5cm \%   after Step 4, we only need to check whether ${\bf u}_{r-2}$, ${\bf u}_{r-1}$ and ${\bf u}_r$ are 
\STATE       \hskip 5cm \%   linearly independent before  updating the last three columns of $V$.
%\STATE 35.~~~~set $3i-2:=r-2$, $3i-1:=r-1$, $3i:=r$, compute ${{\bf v}}_{r-2}$, ${{\bf v}}_{r-1}$, ${{\bf v}}_{r}$
%               via the above Steps 16--32.
%\STATE 36.~\textbf{end if}
%\STATE 37.~\textbf{If} ${\tt mod}(r,3)=2$, \textbf{then} 

\STATE
\STATE        \hskip 5cm \% In  the case ${\tt mod}(r,3)=2$, ${\bf u}_{r-2}\not= 0$ after Step 4, we only need to check 
\STATE        \hskip 5cm \%   whether ${\bf u}_{r-2}$ and ${\bf u}_{r-1}$, and  ${\bf u}_{r-2}$, ${\bf u}_{r-1}$ and ${\bf u}_r$ 
                            are linearly independent
\STATE        \hskip 5cm \%   before updating the last three columns of $V$.
%\STATE 38.~~~~set $3i-2:=r-2$, $3i-1:=r-1$, $3i:=r$, compute ${{\bf v}}_{r-2}$, ${{\bf v}}_{r-1}$, ${{\bf v}}_{r}$
%                via the above Steps 9--32.
%\STATE 39.~\textbf{end if}
\STATE 8.~Replace $U$ with $V$ and $V$ with $U$, $A$ with $A^T$, repeat Steps 3--7.
\STATE 9.~\textbf{Until} stopping criterion
\end{algorithmic}
\end{algorithm}




==> ranknnls_June2.tex <==

\section{A Rank-$k$ NLS based NMF Framework}\label{sec2}
\setcounter{equation}{0}
\smallskip


In this section, we present an alternating \emph{rank-k} nonnegative least squares framework for NMF (\ref{nmf}).

For NMF (\ref{nmf}), suppose that $U$ and $V$ are partitioned into
\begin{equation}\label{UV}
 U=  \left[ \begin{array}{ccc} U_1 & \cdots & U_q  \end{array}\right], \qquad
   V=  \left[ \begin{array}{ccc} V_1 & \cdots & V_q  \end{array}\right], \qquad
   U_1, \cdots, U_q\in \mathbb{R}^{m\times k}, \quad
   V_1, \cdots, V_q\in \mathbb{R}^{n\times k}.
\end{equation}
Then
\[ f(U, V)=f(U_1, \cdots, U_q, V_1, \cdots, V_q):= \|A-UV^T\|^2_F
    =\| U_1V_1^T+\cdots+U_qV_q^T-A\|_F^2. \]
Following the BCD scheme \cite{KHP}, $f$ can be minimized by iteratively solving
\begin{equation}\label{V}
  V_i=\arg \min_{\mathcal{Y} \geq 0} f(U_1, \cdots, U_q, V_1, \cdots, V_{i-1}, \mathcal{Y},  V_{i+1}, \cdots, V_q) 
     =\arg \min_{\mathcal{Y}\geq 0} \| U_i\mathcal{Y}^T-(A-\sum_{l\not= i} U_lV_l^T)\|_F^2
\end{equation}
for $i=1, \cdots, q$, and
\begin{equation}\label{U}
  U_i=\arg \min_{\mathcal{Y}\geq 0} f(U_1, \cdots, U_{i-1}, \mathcal{Y}, U_{i+1}, \cdots, U_q, V_1, \cdots, V_q)
     =\arg \min_{\mathcal{Y}\geq 0} \| V_i \mathcal{Y}^T-(A-\sum_{l\not=i} U_lV_l^T)^T\|_F^2  
\end{equation}
for $i=1, \cdots, q$.  These subproblems are of the form
\begin{equation}\label{gnmf}
 \min_{Y\geq 0} \|GY- B\|_F^2
\end{equation}
with $Y=\mathcal{Y}^T$, and
\[  G=U_i, \ B=A-\sum_{l\neq i}U_lV_l^T, \quad {\rm or } \quad G=V_i, \ B=(A-\sum_{l\neq i}U_lV_l^T)^T, \]
for $i=1, \cdots, q$.


As we will show in the following Theorem, a promising aspect of the $2q$ block partitioning (\ref{UV}) of 
the NMF (\ref{nmf}) is that the  subproblem (\ref{gnmf}) and  so subproblems (\ref{V}) and (\ref{U}) have a closed-form solution.

\begin{theorem}\label{thm1-coro}
Given $ {B} \in \mathbb{R}^{m\times n}$, $ {G} \in \mathbb{R}^{m\times k}$ and ${\bf g}_{k+1}\in \mathbb{R}^m$.
Assume that ${G}$ and $\left[ \begin{array}{cc} G & {\bf g}_{k+1}\end{array}\right]$ are of full column rank.
Denote the unique solution  of the \emph{rank-k NLS} problem (\ref{gnmf}) by $ {S}({G}, {B}) \in \mathbb{R}^{k\times n}$.
Then the unique solution of the \emph{rank-(k+1) NLS} problem
\begin{eqnarray}\label{gn5}
\left[ \begin{array}{c}  {Y}^{\star} \\  {\bf y}_{k+1}^{\star}\end{array}\right]=\arg
\min_{ {Y} \geq 0, {\bf y}_{k+1}\geq 0}
    \| \left[ \begin{array}{cc} {G} & {\bf g}_{k+1} \end{array}\right]
     \left[ \begin{array}{c} {Y} \\ {\bf y}_{k+1} \end{array}\right]-{B} \|_F^2
\end{eqnarray}
is given by
\begin{eqnarray*}
\begin{cases}
{\bf y}_{k+1}^{\star}&=\frac{1}{\|{\bf g}_{k+1}\|^2}  \big[  {\bf g}^T_{k+1}
\big( {B} - {G} \cdot
      {S}({G}-\frac{{\bf g}_{k+1}{\bf g}_{k+1}^T}{\|{\bf g}_{k+1}\|^2} {G},
      {B}-\frac{ {\bf g}_{k+1} {\bf g}_{k+1}^T }{\|{\bf g}_{k+1}\|^2} {B}) \big)
      \big]_+ \in \mathbb{R}^{1\times n}, \\
 {Y}^{\star}&={S}({G}, {B}-{\bf g}_{k+1} {\bf y}^*_{k+1}).
\end{cases}
\end{eqnarray*}
\end{theorem}

\begin{proof} Theorem \ref{thm1-coro} is trivially from Theorem \ref{thm1} which is proved in the next section. \end{proof}

Theorem \ref{thm1-coro} enables us to derive the closed form solution of the \emph{rank-k NLS} problem (\ref{gnmf})
and so subproblems (\ref{V}) and (\ref{U}). It yields the alternating \emph{rank-k} nonnegative
least squares framework called ARkNLS for NMF (\ref{nmf}) in Algorithm \ref{alg1-1}.

\begin{algorithm}%[H]
\caption{An Alternating \emph{rank-k} Nonnegative Least Squares Framework for NMF  (ARkNLS)} \label{alg1-1}
\begin{algorithmic}
\STATE 1.~Given $A \in \mathbb{R}^{m\times n}$.
Initialize $U\in \mathbb{R}^{m\times r}$, $V\in \mathbb{R}^{n\times r}$ with $U, V\geq 0$ and partitioning (\ref{UV}) and
normalized the columns of $U$.
\STATE 2.~\textbf{Repeat}
\STATE 3. Update $V_i$ $(i=1, \cdots, q)$ by solving \emph{rank-k NLS} problems (\ref{V}),
\STATE 4. Update $U_i$ $(i=1, \cdots, q)$ by solving \emph{rank-k NLS} problems (\ref{U}),
\STATE 5.~\textbf{Until} stopping criterion
\end{algorithmic}
\end{algorithm}


According to Theorem 1 in  \cite{KHP}, which characterizes the convergence property of the BCD scheme, the convergence property
of ARkNLS can be stated as follows.

\begin{theorem}\label{thm-convergence} If $U_i$ and $V_i$ are of full column rank for $i=1, \cdots, q$ throughout
all the iterations and the minimums in (\ref{V}) and (\ref{U}) are attained at each updating step, every limit point
of the sequence $\{ (U,~V)^{(i)} \}$ generated by ARkNLS algorithm is a stationary point of the NMF (\ref{nmf}).
\end{theorem}


It is obvious that ARkNLS is a general framework in which we can choose any $k$ we want.
It covers HALS, ANLS, and other possible $k$ values we will propose since when
$k=1$ it is HALS and  when $k=r$ it is ANLS.




\section{Recursive Formula for the Solution of \emph{Rank-k NLS} Problem}\label{sec3}
\setcounter{equation}{0}
\smallskip

Problem  (\ref{gnmf}) (and so problems (\ref{V}) and (\ref{U})) can be decoupled into independent NLS problems with single right-hand side vector as
\[ \min_{{Y}(:, j) \in \mathbb{R}^{k \times 1},
                                     {Y}(:, j)\geq 0}
                       \|G  {Y}(:, j)-{B}(: j)\|_F^2.
\]
As a result, in order to derive the closed-form solution of the \emph{rank-k NLS} problem (\ref{gnmf}) (and so problems (\ref{V}) and (\ref{U})),
in the following we first establish the recursive formula for the solution of the \emph{rank-k NLS} problem (\ref{n4}) with 
the following compact form:
\begin{eqnarray}\label{n4}
\min_{{\bf y}\geq{\bf 0}} \|G{\bf y}-{\bf b}\|,
\end{eqnarray}
where ${\bf b}\in \mathbb{R}^m$, $G\in \mathbb{R}^{m\times k}$, and ${\rm rank} (G) =k$.


\begin{Lemma}\label{lem0}
Given a continuous and  convex function $f({\bf z})$, and two nonempty closed convex sets $\mathcal{T}$ and $\mathcal{C}$
satisfying $\mathcal{T}\cap\mathcal{C}\neq\emptyset$. Assume
\[ \widetilde{\bf z}={\rm arg} \min_{{\bf z}\in \mathcal{T}} f({\bf z}),
\]
and $\widetilde{\bf z}$ is finite.
Assume further that the following constrained optimization problem
\begin{eqnarray}\label{n1}
\min_{{\bf z}\in \mathcal{T}\cap\mathcal{C}} f({\bf z})
\end{eqnarray}
has a finite solution.


1) If $\widetilde{\bf z}\in \mathcal{C}$, then
\[ {\bf z}^*=\widetilde{\bf z}={\rm arg} \min_{{\bf z}\in \mathcal{T}\cap\mathcal{C}} f({\bf z}). \]

2) If $\widetilde{\bf z}\notin \mathcal{C}$, then there exists a ${\bf {z}}^*\in\mathcal{T}\cap\mathcal{C}_{edge}$ satisfying
\[ {\bf {z}}^*={\rm arg} \min_{{\bf z}\in \mathcal{T}\cap\mathcal{C}} f({\bf z}), \]
where $\mathcal{C}_{edge}$ denotes the boundary of $\mathcal{C}$.
\end{Lemma}

\begin{proof} Part 1) is obvious. In the following we  prove Part 2).

Let ${\bf \widehat{z}}\in\mathcal{T}\cap\mathcal{C}$ be finite and
\begin{equation} {\bf \widehat{z}}={\rm arg} \min_{\mathcal{T}\cap\mathcal{C}} f({\bf z}). \label{*}
\end{equation}
It is clear that Part 2) follows with ${\bf {z}}^*={\bf \widehat{z}}$ if
${\bf \widehat{z}}\in\mathcal{T}\cap\mathcal{C}_{edge}$.
Otherwise, suppose that
${\bf \widehat{z}}\in\mathcal{T}\cap\mathcal{C}_{int}$,  where $\mathcal{C}_{int}$ is the interior of $\mathcal{C}$.
 Note that $\widetilde {\bf z}\notin \mathcal{C}$, $\widetilde{\bf z}\in \mathcal{T}$ and
 ${\bf \widehat{z}}\in \mathcal{T}\cap\mathcal{C}_{int}$.
Therefore, there exists
${\bf {z}}^* \in\mathcal{T}\cap\mathcal{C}_{edge}$
such that for some $t\in(0,1)$, we have
\[ {\bf {z}}^*=(1-t) \widetilde{\bf z}+t{\bf \widehat{z}}\in \mathcal{T}\cap\mathcal{C}_{edge}. \]
Furthermore,
\[ f(\widetilde{\bf z})\leq f(\widehat{\bf z}). \]
Hence,
\[ %\label{n2}
f({\bf {z}}^*)\leq(1-t)f(\widetilde{\bf z})+t f({\bf \widehat{z}})\leq(1-t)f({\bf \widehat{z}})+tf({\bf \widehat{z}})
       =f({\bf \widehat{z}}),
\]
which together with (\ref{*}) yields that
\[ f({\bf {z}}^*)=f({\bf \widehat{z}}), \]
and thus,
\[ {\bf {z}^*}={\rm arg} \min_{{\bf z}\in \mathcal{T}\cap\mathcal{C}} f({\bf z}). \]
\end{proof}


\begin{Lemma}\label{lem*}
Assume that ${\bf b}\in \mathbb{R}^m$, $G\in \mathbb{R}^{m\times k}$,
and ${\rm rank} (G) =k$. Then the  solution  of the \emph{rank-k NLS} problem (\ref{n4}) is unique.
\end{Lemma}

\begin{proof} The proof is trivial and thus is omitted here.
\end{proof}

Now, we establish the recursive formula for the solution of \emph{rank-k NLS} problem (\ref{n4}).

\begin{theorem}\label{thm1}
Given ${\bf b}\in \mathbb{R}^m$, $G\in \mathbb{R}^{m\times k}$ and ${\bf g}_{k+1}\in \mathbb{R}^m$.
Assume that $G$ and and $\left[ \begin{array}{cc} G & {\bf g}_{k+1}\end{array}\right]$ are of full column rank.
Denote the unique solution  of the \emph{rank-k NLS} problem (\ref{n4}) by $s(G, {\bf b}) \in \mathbb{R}^k$.
Then the unique solution of the \emph{rank-(k+1) NLS} problem
\begin{eqnarray}\label{n5}
\left[ \begin{array}{c} {\bf y}^{\star} \\  y_{k+1}^{\star}\end{array}\right]= \arg
    \min_{{\bf y}\geq{\bf 0},y_{k+1}\geq0} \|(G{\bf y}+{\bf g}_{k+1}y_{k+1})-{\bf b}\|
\end{eqnarray} is given by
\begin{eqnarray*}
\begin{cases}
y_{k+1}^{\star}&=\frac{1}{\|{\bf g}_{k+1}\|^2}\big[{\bf g}^T_{k+1}\big({\bf b}-G\cdot
s(G-\frac{{\bf g}_{k+1}{\bf g}_{k+1}^T}{\|{\bf g}_{k+1}\|^2} G, {\bf b}-\frac{{\bf g}_{k+1} {\bf g}_{k+1}^T }{\|{\bf g}_{k+1}\|^2} {\bf b}))
\big]_+, \\
{\bf y}^{\star}&=s(G, {\bf b}-{\bf g}_{k+1}y^*_{k+1}).
\end{cases}
\end{eqnarray*}
\end{theorem}

\begin{proof}
We first consider the optimization problem
\begin{eqnarray}\label{n6}
\min_{{\bf y}\geq{\bf 0}} \|(G{\bf y}+{\bf g}_{k+1}y_{k+1})-{\bf b}\|.
\end{eqnarray}
Obviously, for any given ${\bf y}$, the solution $y_{k+1}$ to the problem \eqref{n6} is uniquely given by
\[ y_{k+1}=\frac{{\bf g}^T_{k+1}({\bf b}-G{\bf y})}{\|{\bf g}_{k+1}\|^2}.\]
So, the optimization problem \eqref{n6} reduces to
\begin{eqnarray}\label{n7}
\min_{{\bf y}\geq{\bf 0}} \|(G{\bf y}+{\bf g}_{k+1}\frac{{\bf g}^T_{k+1}({\bf b}-G{\bf y})}{\|{\bf g}_{k+1}\|^2})-{\bf b}\|
      =\min_{{\bf y}\geq{\bf 0}}\|\widetilde{G}{\bf y}-{\bf \widetilde{b}}\|,
\end{eqnarray}
where
\[ {\bf \widetilde{b}}={\bf b}-\frac{{\bf g}_{k+1}{\bf g}^T_{k+1}}{\|{\bf g}_{k+1}\|^2}{\bf b}, \quad
 \widetilde{G}=G-\frac{{\bf g}_{k+1}{\bf g}^T_{k+1}}{\|{\bf g}_{k+1}\|^2}G,
\]
and $\widetilde{G}$ is of full column rank.
The unique solution $\widetilde{\bf y}$ of the problem (\ref{n7}) is $s(\widetilde{G}, {\bf \widetilde{b}})$.
Therefore, the unique solution to the problem \eqref{n6} is given by
\begin{eqnarray*}
\widetilde y_{k+1} &=& \frac{{\bf g}^T_{k+1}({\bf b}-G\cdot s(\widetilde{G}, {\bf \widetilde{b}}))}{\|{\bf g}_{k+1}\|^2}, \\
\widetilde {\bf y} &=& s(G, {\bf b}-{\bf g}_{k+1} \widetilde y_{k+1}).
\end{eqnarray*}
Let
\[ \mathcal{T}:=\{ \left[ \begin{array}{c} {\bf y} \\ y_{k+1} \end{array}\right] |~{\bf y}\in \mathbb{R}^k, ~{\bf y}\geq0\}, \qquad
\mathcal{C}:=\{ \left[ \begin{array}{c} {\bf y} \\ y_{k+1} \end{array}\right] |~{\bf y}\in \mathbb{R}^k, ~{\bf y}\geq0, ~y_{k+1}\geq 0\}. \]
By Lemma \ref{lem0},
\begin{itemize}
\item if $\widetilde y_{k+1}\geq0$, then $\left[ \begin{array}{c} {\bf y}^{\star} \\  y_{k+1}^{\star}\end{array}\right]$ with
\begin{eqnarray*}
y^*_{k+1} &=& \widetilde y_{k+1} = \frac{{\bf g}^T_{k+1}({\bf b}-G\cdot s(\widetilde{G}, {\bf \widetilde{b}}))}{\|{\bf g}_{k+1}\|^2}
=\frac{[{\bf g}^T_{k+1}({\bf b}-G\cdot s(\widetilde{G}, {\bf \widetilde{b}}))]_+}{\|{\bf g}_{k+1}\|^2}, \\
{\bf y}^{\star} &=& \widetilde {\bf y} = s(G, {\bf b}-{\bf g}_{k+1} \widetilde y_{k+1})
   =s(G, {\bf b}-{\bf g}_{k+1} y^*_{k+1}),
\end{eqnarray*}
is the unique solution of the problem \eqref{n5};
\item if $\widetilde y_{k+1}<0$, then the unique solution $y_{k+1}$ of the problem  \eqref{n5} is
$$ y^{\star}_{k+1}=0=\frac{[{\bf g}^T_{k+1}({\bf b}-G\cdot s(\widetilde{G}, {\bf \widetilde{b}}))]_+}{\|{\bf g}_{k+1}\|^2}, $$
and consequently, the unique solution ${\bf y}$ of the problem \eqref{n5} is given by
\[ {\bf y}^{\star}=s(G, {\bf b}-{\bf g}_{k+1}y^*_{k+1}). \]
\end{itemize}

\end{proof}


Theorem \ref{thm1} can be used to derive the closed-form solution of the \emph{rank-k NLS} problem (\ref{n4}) for any integer $k\geq 1$.
As an example, we give the closed-form solutions of the \emph{rank-2 NLS} and \emph{rank-3 NLS} in the following two corollaries.

\begin{corollary}\label{cor1}
Assume that $G=\left[ \begin{array}{cc} {\bf g}_1 & {\bf g}_2\end{array}\right]\in \mathbb{R}^{m\times 2}$ is of full column rank.
Then the unique solution of the  \emph{rank-2 NLS} problem
\begin{align}\label{n10}
\left[ \begin{array}{c} y_1^* \\  y_2^*\end{array}\right]=\arg \min_{{\bf y}\geq0}\|G{\bf y}-{\bf b}\|=
{\rm arg} \min_{\{y_1,y_2\}\geq0}\|y_1{\bf g}_1+y_2{\bf g}_2-{\bf b}\|
\end{align}
is given by
\begin{eqnarray}\label{n9}
\begin{cases}
y_2^*&=\frac{1}{\|{\bf g}_2\|^2}\left[{\bf b}^T{\bf g}_2-{\bf g}^T_2{\bf g}_1
       \left[\frac{\|{\bf g}_2\|^2{\bf b}^T{\bf g}_1-{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1}{ \|{\bf g}_1\|^2\|{\bf g}_2\|^2
        -({\bf g}_1^T{\bf g}_2)^2  } \right]_{+}\right]_{+}\\
y_1^*&=\frac{1}{\|{\bf g}_1\|^2}[{\bf b}^T{\bf g}_1-({\bf g}^T_2{\bf g}_1)y_2^*]_{+}.
\end{cases}
\end{eqnarray}
\end{corollary}

\begin{proof}
Since  the solution of the \emph{rank-1 NLS} problem
\[ %\label{n11}
\min_{y_1\geq0}\|y_1{\bf g}_1-{\bf b}\|
\]
is given by
\[s({\bf g}_1, {\bf b})= \frac{[{\bf g}^T_1{\bf b}]_+}{\|{\bf g}_1\|^2}, \]
according to Theorem \ref{thm1}, the solution $y_2^*$ to \emph{rank-2 NLS} problem \eqref{n10} is
$$y^*_2=\frac{\big[{\bf g}^T_{2}({\bf b}-{\bf g}_1\cdot
s({\bf g}_1-\frac{{\bf g}_{2}{\bf g}^T_{2}}{\|{\bf g}_{2}\|^2}{\bf g}_1, {\bf b}-\frac{{\bf g}_{2}{\bf g}^T_{2}}{\|{\bf g}_{2}\|^2}{\bf b})\big]_+}{\|{\bf g}_{2}\|^2}.$$
Note that
\begin{eqnarray*}
s({\bf g}_1-\frac{{\bf g}_{2}{\bf g}^T_{2}}{\|{\bf g}_{2}\|^2}{\bf g}_1, {\bf b}-\frac{{\bf g}_{2}{\bf g}^T_{2}}{\|{\bf g}_{2}\|^2}{\bf b})
&=& \frac{\big[\big({\bf g}_1-{\bf g}_{2}\frac{{\bf g}^T_{2}{\bf g}_1}{\|{\bf g}_{2}\|^2}\big)^T\big({\bf b}-{\bf g}_{2}\frac{{\bf g}^T_{2}{\bf b}}{\|
{\bf g}_{2}\|^2}\big)\big]_+}{\left\|{\bf g}_1-{\bf g}_{2}\frac{{\bf g}^T_{2}{\bf g}_1}{\|{\bf g}_{2}\|^2}\right\|^2} \\
&=& \frac{\left[\|{\bf g}_2\|^2{\bf b}^T{\bf g}_1-{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1\right]_{+}}
{  \|{\bf g}_1\|^2\|{\bf g}_2\|^2-({\bf g}_1^T{\bf g}_2)^2 },
\end{eqnarray*}
then
\begin{eqnarray*}
\begin{cases}
y^*_2&=\frac{1}{\|{\bf g}_2\|^2}\left[{\bf b}^T{\bf g}_2-{\bf g}^T_2{\bf g}_1\left[\frac{\|{\bf g}_2\|^2{\bf b}^T{\bf g}_1
      -{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1}{ \|{\bf g}_1\|^2\|{\bf g}_2\|^2-({\bf g}_1^T{\bf g}_2)^2  }\right]_{+}\right]_{+}\\
y^*_1&=\frac{1}{\|{\bf g}_1\|^2}[{\bf b}^T{\bf g}_1-({\bf g}^T_2{\bf g}_1)y_2^*]_{+},
\end{cases}
\end{eqnarray*}
and (\ref{n10}) holds. \end{proof}

\begin{corollary}\label{cor2}
Assume that $G=\left[ \begin{array}{ccc} {\bf g}_1 & {\bf g}_2 &  {\bf g_3} \end{array}\right]\in \mathbb{R}^{m\times 3}$
is of full column rank. Then the unique solution of the \emph{rank-3 NLS} problem
\begin{align*}
  \left[ \begin{array}{c} y^*_1 \\ y^*_2 \\ y^*_3\end{array}\right]={\rm arg}
  \min_{{\bf y}\geq0}\|G{\bf y}-{\bf b}\|
 = {\rm arg} \min_{\{y_1,y_2,y_3\} \geq0}\|y_1{\bf g}_1+y_2{\bf g}_2+y_3{\bf g}_3-{\bf b}\|
\end{align*}
is given by \begin{align}\label{r3}
\begin{cases}
y^*_3&=\frac{1}{\|{\bf g}_3\|^2}[{\bf b}^T{\bf g}_3-({\bf g}^T_3{\bf g}_1)\widetilde{p}-({\bf g}^T_3{\bf g}_2)p]_{+}\\
y^*_2&=\frac{1}{\|{\bf g}_2\|^2}\left[{\bf b}^T{\bf g}_2-({\bf g}_3^T{\bf g}_2)y^*_3-{\bf g}^T_2{\bf g}_1\big[\frac{({\bf b}^T{\bf g}_1\|
                  {\bf g}_2\|^2-{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1)- ({\bf g}^T_3{\bf g}_1\|{\bf g}_2\|^2
                   -{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1)y^*_3}{\|{\bf g}_1\|^2\|{\bf g}_2\|^2-({\bf g}^T_2
                   {\bf g}_1)^2}\big]_{+}\right]_{+}\\
y^*_1&=\frac{1}{\|{\bf g}_1\|^2}[{\bf b}^T{\bf g}_1-({\bf g}^T_3{\bf g}_1)y^*_3-({\bf g}^T_2{\bf g}_1)y^*_2]_{+},
\end{cases}
\end{align}
where
\begin{eqnarray*}\label{q1}
p=\left[\frac{{\bf b}^T{\bf g}_2\cdot\|{\bf g}_3\|^2-{\bf b}^T{\bf g}_3\cdot{\bf g}^T_3{\bf g}_2}{\|{\bf g}_2\|^2\|{\bf g}_3\|^2
         -({\bf g}^T_3{\bf g}_2)^2}-\frac{{\bf g}^T_2{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_3{\bf g}_1}{\|
          {\bf g}_2\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)^2}\big[\frac{{\rm det}([{\bf b},{\bf g}_2,{\bf g}_3]^TG)}
           {{\rm det}(G^TG)}\big]_{+}\right]_{+},
\end{eqnarray*}
and
\begin{eqnarray*}\label{q2}
\widetilde{p}=\left[\frac{{\bf b}^T{\bf g}_1\cdot\|{\bf g}_3\|^2
                      -{\bf b}^T{\bf g}_3\cdot{\bf g}^T_3{\bf g}_1}{\|{\bf g}_1\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)^2}
                      -\frac{{\bf g}^T_2{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_3{\bf g}_1}{\|{\bf g}_1\|^2\|
                      {\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)^2}p\right]_{+}.
\end{eqnarray*}
\end{corollary}

\begin{proof}
Let
$${\bf \widehat{b}}={\bf b}-\frac{{\bf g}_{3}{\bf g}^T_{3}}{\|{\bf g}_{3}\|^2}{\bf b},~~
{\bf \widehat{g}}_1={\bf g}_{1}-\frac{{\bf g}_{3}{\bf g}^T_{3}}{\|{\bf g}_{3}\|^2}{\bf g}_{1},~~
{\bf \widehat{g}}_2={\bf g}_{2}-\frac{{\bf g}_{3}{\bf g}^T_{3}}{\|{\bf g}_{3}\|^2}{\bf g}_{2},~~
 $$
A simple calculation yields that
\begin{align}
{\bf \widehat{g}}^T_2{\bf \widehat{g}}_1
&=({\bf g}_{2}-\frac{{\bf g}^T_{3}{\bf g}_{2}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{1}
              -\frac{{\bf g}^T_{3}{\bf g}_{1}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{({\bf g}^T_2{\bf g}_1)\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)({\bf g}^T_3{\bf g}_1)}{\|{\bf g}_{3}\|^2},\label{n18}\\
\|{\bf \widehat{g}}_1\|^2
&=({\bf g}_{1}-\frac{{\bf g}^T_{3}{\bf g}_{1}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{1}
              -\frac{{\bf g}^T_{3}{\bf g}_{1}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{\|{\bf g}_1\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)^2}{\|{\bf g}_{3}\|^2},\label{n21}\\
\|{\bf \widehat{g}}_2\|^2
&=({\bf g}_{2}-\frac{{\bf g}^T_{3}{\bf g}_{2}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{2}
              -\frac{{\bf g}^T_{3}{\bf g}_{2}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{\|{\bf g}_2\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)^2}{\|{\bf g}_{3}\|^2},\label{n16}\\
{\bf \widehat{b}}^T{\bf \widehat{g}}_2
&=({\bf b}-\frac{{\bf g}^T_{3}{\bf b}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{2}
         -\frac{{\bf g}^T_{3}{\bf g}_{2}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{({\bf b}^T{\bf g}_2)\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)({\bf g}^T_3{\bf b})}{\|{\bf g}_{3}\|^2},\label{n17}\\
{\bf \widehat{b}}^T{\bf \widehat{g}}_1
&=({\bf b}-\frac{{\bf g}^T_{3}{\bf b}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{1}
          -\frac{{\bf g}^T_{3}{\bf g}_{1}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{({\bf b}^T{\bf g}_1)\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)({\bf g}^T_3{\bf b})}{\|{\bf g}_{3}\|^2}.\label{n19}
\end{align}
Let $s(\left[ \begin{array}{cc} {\bf {\widehat g}}_1 & {\bf {\widehat g}}_2 \end{array}\right], {\bf {\widehat b}})
     =\left[
     \begin{array}{c}
          s_1(\left[ \begin{array}{cc} {\bf {\widehat g}}_1 & {\bf {\widehat g}}_2 \end{array}\right], {\bf {\widehat b}}) \\
          s_2(\left[ \begin{array}{cc} {\bf {\widehat g}}_1 & {\bf {\widehat g}}_2 \end{array}\right], {\bf {\widehat b}}) \\
     \end{array}
     \right]$
be the solution to the optimization problem
\[ \min_{y_1,y_2\geq0}\|y_1{\bf {\widehat g}}_1+y_2{\bf {\widehat g}}_2-{\bf {\widehat b}}\|. \]
Then from \eqref{n18}--\eqref{n19} and Corollary \ref{cor1}, we have
\begin{align*}
s_2(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})
&=\frac{1}{\|{\bf \widehat{g}}_2\|^2}\left[{\bf \widehat{b}}^T{\bf \widehat{g}}_2
             -{\bf \widehat{g}}^T_2{\bf \widehat{g}}_1\left[\frac{\|{\bf \widehat{g}}_2\|^2{\bf \widehat{b}}^T{\bf \widehat{g}}_1
             -{\bf \widehat{b}}^T{\bf \widehat{g}}_2\cdot{\bf \widehat{g}}^T_2{\bf \widehat{g}}_1}{\|{\bf \widehat{g}}_1\|^2\|{\bf \widehat{g}}_2\|^2-({\bf \widehat{g}}_1^T{\bf \widehat{g}}_2)^2}\right]_{+}\right]_{+}\nonumber\\
&=\left[\frac{{\bf b}^T{\bf g}_2\cdot\|{\bf g}_3\|^2-{\bf b}^T{\bf g}_3\cdot{\bf g}^T_3{\bf g}_2}{\|{\bf g}_2\|^2\|{\bf g}_3\|^2
             -({\bf g}^T_3{\bf g}_2)^2}-\frac{{\bf g}^T_2{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_3{\bf g}_1}
              {\|{\bf g}_2\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)^2}\big[\frac{{\rm det}([{\bf b},{\bf g}_2,{\bf g}_3]^TG)}
               {{\rm det}(G^TG)}\big]_{+}\right]_{+} \nonumber \\
&=p.
\end{align*}
Moreover,
\begin{eqnarray*}
s_1(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})
&=& \left[\frac{{\bf b}^T{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf b}^T{\bf g}_3\cdot{\bf g}^T_3{\bf g}_1}{\|{\bf g}_1\|^2\|{\bf g}_3\|^2
            -({\bf g}^T_3{\bf g}_1)^2}-\frac{{\bf g}^T_2{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_3{\bf g}_1}
               {\|{\bf g}_1\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)^2}
s_2(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right],
{\bf \widehat{b}})\right]_{+}\\
&=&\widetilde p.
\end{eqnarray*}
Therefore, according to Theorem \ref{thm1} and Corollary \ref{cor1}, the solution to the optimization problem
\[ \min_{y_1,y_2,y_3\geq0}\|y_1{\bf g}_1+y_2{\bf g}_2+y_3{\bf g}_3-{\bf b}\| \]
is
\begin{eqnarray*}
y^*_3 &=& \frac{1}{\|{\bf g}_{3}\|^2}\big[{\bf g}^T_{3}\big({\bf b}-[{\bf g}_1,{\bf g}_2]\cdot
s( \left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})\big)\big]_+ \\
%&=&\frac{1}{\|{\bf g}_{3}\|^2}\big[{\bf g}^T_{3}{\bf b}-{\bf g}^T_{3}{\bf g}_1\cdot
%s_1(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})
%-{\bf g}^T_{3}{\bf g}_2\cdot
%s_2(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})\big]_+,\\
&=&\frac{1}{\|{\bf g}_{3}\|^2}\big[{\bf g}^T_{3}{\bf b}-{\bf g}^T_{3}{\bf g}_1\cdot \widetilde{p}
-{\bf g}^T_{3}{\bf g}_2\cdot p\big]_+,
\end{eqnarray*}
with $s_1(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})=\widetilde{p}$, $s_2(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})=p$,
and
\begin{align*}
\begin{cases}
y^*_2&=s_2( \left[ \begin{array}{cc} {\bf g}_1 & {\bf g}_2 \end{array}\right],  {\bf b}-{\bf g}_{3}y^*_{3})\\
~&=\frac{1}{\|{\bf g}_2\|^2}\left[({\bf b}-{\bf g}_{3}y^*_{3})^T{\bf g}_2-{\bf g}^T_2{\bf g}_1\left[\frac{\|{\bf g}_2\|^2({\bf b}
       -{\bf g}_{3}y^*_{3})^T{\bf g}_1-({\bf b}-{\bf g}_{3}y^*_{3})^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1}{\|{\bf g}_1\|^2\|{\bf g}_2\|^2
       -({\bf g}^T_2{\bf g}_1)^2}\right]_{+}\right]_{+}\\
~&=\frac{1}{\|{\bf g}_2\|^2}\left[({\bf b}-{\bf g}_3y^*_3)^T{\bf g}_2-{\bf g}^T_2{\bf g}_1\big[\frac{({\bf b}^T{\bf g}_1\|{\bf g}_2\|^2
       -{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1)- ({\bf g}^T_3{\bf g}_1\|{\bf g}_2\|^2
       -{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1)y^*_3}{\|{\bf g}_1\|^2\|{\bf g}_2\|^2
       -({\bf g}^T_2{\bf g}_1)^2}\big]_{+}\right]_{+}\\
y^*_1&=s_1(\left[ \begin{array}{cc} {\bf g}_1 & {\bf g}_2\end{array}\right], {\bf b}-{\bf g}_{3}y^*_{3})
=\frac{1}{\|{\bf g}_1\|^2}[({\bf b}-{\bf g}_{3}y^*_{3})^T{\bf g}_1-({\bf g}^T_2{\bf g}_1)y^*_2]_{+}.
\end{cases}
\end{align*}
Hence, Corollary \ref{cor2} is proved.
\end{proof}



==> ranknnls_June3.tex <==

\section{ARkNLS: a Rank-$k$ NLS based NMF Framework}\label{sec2}
\setcounter{equation}{0}
\smallskip


In this section, we present a framework called ARkNLS (alternating \emph{rank-k} nonnegative least squares) for NMF (\ref{nmf}). ARkNLS represents a set of block coordinate descent methods for NMF where a block consists of $k$ columns of $U$ or $k$ columns of $V$.
Specifically, for NMF (\ref{nmf}), 
suppose ${U}^* \in \mathbb{R}^{m\times r}$ and ${V}^* \in \mathbb{R}^{n\times r}$ 
are partitioned  as follows:
\begin{equation}\label{UV}
 U=  \left[ \begin{array}{ccc} U_1 & \cdots & U_q  \end{array}\right], \qquad
   V=  \left[ \begin{array}{ccc} V_1 & \cdots & V_q  \end{array}\right], \qquad
   U_1, \cdots, U_q\in \mathbb{R}^{m\times k}, \quad
   V_1, \cdots, V_q\in \mathbb{R}^{n\times k}.
\end{equation}
For simplicity of discussion, let us assume that $r/k=q$ is an integer, for now.
Later, we will show how the cases can be handled when $r$ is not divisible by $k$.
We have
\[ f(U, V)=f(U_1, \cdots, U_q, V_1, \cdots, V_q):= \|A-UV^T\|^2_F
    =\| U_1V_1^T+\cdots+U_qV_q^T-A\|_F^2. \]
Following the BCD scheme \cite{KHP}, $f$ can be minimized by iteratively solving\\
For $i=1, \cdots, q$, 
\begin{equation}\label{V}
  V_i=\arg \min_{\mathcal{Y} \geq 0} f(U_1, \cdots, U_q, V_1, \cdots, V_{i-1}, \mathcal{Y},  V_{i+1}, \cdots, V_q) 
     =\arg \min_{\mathcal{Y}\geq 0} \| U_i\mathcal{Y}^T-(A-\sum_{l\not= i} U_lV_l^T)\|_F^2
\end{equation}
and for $i=1, \cdots, q$, 
\begin{equation}\label{U}
  U_i=\arg \min_{\mathcal{Y}\geq 0} f(U_1, \cdots, U_{i-1}, \mathcal{Y}, U_{i+1}, \cdots, U_q, V_1, \cdots, V_q)
     =\arg \min_{\mathcal{Y}\geq 0} \| V_i \mathcal{Y}^T-(A-\sum_{l\not=i} U_lV_l^T)^T\|_F^2  
\end{equation}

The above yields the alternating \emph{rank-k} nonnegative
least squares framework ARkNLS for NMF (\ref{nmf}) which is summarized 
in Algorithm \ref{alg1-1}.
The proposed ARkNLS is a general framework where we can choose any integer $k$.  
When $k=1$, it represents a $2r$ block BCD and is reduced to HALS.
When $k=r$, it represents a 2 block BCD and ANLS/BPP is one of such algorithm.


\begin{algorithm}[h]
\caption{{\bf ARkNLS}: Alternating \emph{rank-k} Nonnegative Least Squares Framework for NMF} \label{alg1-1}
\begin{algorithmic}
\STATE 1.~Assume $A \in \mathbb{R}^{m\times n}$ and $r \leq \min(m,n)$ are given.\\
Initialize $U\in \mathbb{R}^{m\times r}$ and $V\in \mathbb{R}^{n\times r}$ with $\{U, V\}\geq 0$ \\
Partition as in (\ref{UV}) where each block $U_i$ and $V_i$ has $k$ columns for some integer $k$,
such that $qk = r$. \\
Normalize the columns of $U$.
\STATE 2.~\textbf{Repeat}
\STATE 3. \hspace{0.1in} For $i=1, \cdots, q$, \\
\hspace{0.3in} update $V_i$ by solving \emph{rank-k NLS} problems (\ref{V})
\STATE 4. \hspace{0.1in} For $i=1, \cdots, q$, \\
\hspace{0.3in} update $U_i$ by solving \emph{rank-k NLS} problems (\ref{U})
\STATE 5.~\textbf{Until} stopping criterion is satisfied
\end{algorithmic}
\end{algorithm}

The subproblems (\ref{U}) and (\ref{V}) are NLS with multiple right hand sides, of the form
\begin{equation}\label{gnmf}
 \min_{Y\geq 0} \|GY- B\|_F^2
\end{equation}
%with $Y=\mathcal{Y}^T$, and
where
$ G=U_i$ and $B=A-\sum_{l\neq i}U_lV_l^T$ for $i=1, \cdots, q$
in (\ref{V}).
Likewise
$G=V_i$ and $B=(A-\sum_{l\neq i}U_lV_l^T)^T$ for $i=1, \cdots, q$
in (\ref{U}).
Therefore, an NLS with multiple right hand side vectors (\ref{gnmf})
is the core problem in ARkNLS, which is our focus in this section.

As illustrated in the following theorem, 
a significant aspect of ARkNLS framework is that the NLS (\ref{gnmf}), 
accordingly, the subproblems (\ref{V}) and (\ref{U}) have closed-form solutions.

\begin{theorem}\label{thm1-coro}
Given $ {B} \in \mathbb{R}^{m\times n}$, $ {G} \in \mathbb{R}^{m\times k}$ and ${\bf g}_{k+1}\in \mathbb{R}^m$.
Assume that ${G}$ and $\left[ \begin{array}{cc} G & {\bf g}_{k+1}\end{array}\right]$ are of full column rank.
Denote the unique solution  of the \emph{rank-k NLS} problem (\ref{gnmf}) by $ {S}({G}, {B}) \in \mathbb{R}^{k\times n}$.
Then the unique solution of the \emph{rank-(k+1) NLS} problem
\begin{eqnarray}\label{gn5}
\left[ \begin{array}{c}  {Y}^{\star} \\  {\bf y}_{k+1}^{\star}\end{array}\right]=\arg
\min_{ {Y} \geq 0, {\bf y}_{k+1}\geq 0}
    \| \left[ \begin{array}{cc} {G} & {\bf g}_{k+1} \end{array}\right]
     \left[ \begin{array}{c} {Y} \\ {\bf y}_{k+1} \end{array}\right]-{B} \|_F^2
\end{eqnarray}
is given by
\begin{eqnarray*}
\begin{cases}
{\bf y}_{k+1}^{\star}&=\frac{1}{\|{\bf g}_{k+1}\|^2}  \big[  {\bf g}^T_{k+1}
\big( {B} - {G} \cdot
      {S}({G}-\frac{{\bf g}_{k+1}{\bf g}_{k+1}^T}{\|{\bf g}_{k+1}\|^2} {G},
      {B}-\frac{ {\bf g}_{k+1} {\bf g}_{k+1}^T }{\|{\bf g}_{k+1}\|^2} {B}) \big)
      \big]_+ \in \mathbb{R}^{1\times n}, \\
 {Y}^{\star}&={S}({G}, {B}-{\bf g}_{k+1} {\bf y}^*_{k+1}).
\end{cases}
\end{eqnarray*}
\end{theorem}

\begin{proof} Theorem \ref{thm1-coro} is trivially from Theorem \ref{thm1} which is proved in the next section. \end{proof}

Theorem \ref{thm1-coro} enables us to derive the closed form solution of the \emph{rank-k NLS} problem (\ref{gnmf})
and so subproblems (\ref{V}) and (\ref{U}). 

In addition, according to Theorem 1 in  \cite{KHP}, which characterizes the convergence property of the BCD scheme for NMF, the convergence property
of ARkNLS can be stated as follows.

\begin{theorem}\label{thm-convergence} If $U_i$ and $V_i$ are of full column rank for $i=1, \cdots, q$ throughout
all the iterations and the minimums in (\ref{V}) and (\ref{U}) are attained at each updating step, every limit point
of the sequence $\{ (U,~V)^{(i)} \}$ generated by ARkNLS algorithm is a stationary point of the NMF (\ref{nmf}).
\end{theorem}
It is important to note that for the above theorem to be applicable, we need to have unique
solution for each subproblem when $q>2$ \cite{Grippo and S...}. When any $U_i$ or $V_i$ is rank deficient,
then the uniqueness of the solution will be violated, and therefore, the above theorem cannot
be applied for proof of convergence to a stationary point.
In case of HALS, $q = 2r$ and the uniquess of the solution for all subproblems cannot be guaranteed
since a block $U_i$ or $V_i$ (in case of HALS, these will consist of one vector) may become 
rank deficient (zero vectors).
For NMF algorithms based the BCD scheme with 2 blocks like ANLS/BPP 
(where updates are alternated between blocks
$U$ and $V$), the uniqueness is not required and the convergence result
of the above theorem is applicable.
However, in case of NMF, due to nonuniqueness of the solution, we can modify the subproblems
so that the subproblems are always of full rank and therefore, the solution is unique.
More detailed discussions are presented in Section xxx.





\section{Recursive Formula for the Solution of \emph{Rank-k NLS} Problem}\label{sec3}
\setcounter{equation}{0}
\smallskip

Problem  (\ref{gnmf}) (and so problems (\ref{V}) and (\ref{U})) can be decoupled into independent NLS problems with single right-hand side vector as
\[ \min_{{Y}(:, j) \in \mathbb{R}^{k \times 1},
                                     {Y}(:, j)\geq 0}
                       \|G  {Y}(:, j)-{B}(: j)\|_F^2.
\]
As a result, in order to derive the closed-form solution of the \emph{rank-k NLS} problem (\ref{gnmf}) (and so problems (\ref{V}) and (\ref{U})),
in the following we first establish the recursive formula for the solution of the \emph{rank-k NLS} problem (\ref{n4}) with 
the following compact form:
\begin{eqnarray}\label{n4}
\min_{{\bf y}\geq{\bf 0}} \|G{\bf y}-{\bf b}\|,
\end{eqnarray}
where ${\bf b}\in \mathbb{R}^m$, $G\in \mathbb{R}^{m\times k}$, and ${\rm rank} (G) =k$.


\begin{Lemma}\label{lem0}
Given a continuous and  convex function $f({\bf z})$, and two nonempty closed convex sets $\mathcal{T}$ and $\mathcal{C}$
satisfying $\mathcal{T}\cap\mathcal{C}\neq\emptyset$. Assume
\[ \widetilde{\bf z}={\rm arg} \min_{{\bf z}\in \mathcal{T}} f({\bf z}),
\]
and $\widetilde{\bf z}$ is finite.
Assume further that the following constrained optimization problem
\begin{eqnarray}\label{n1}
\min_{{\bf z}\in \mathcal{T}\cap\mathcal{C}} f({\bf z})
\end{eqnarray}
has a finite solution.


1) If $\widetilde{\bf z}\in \mathcal{C}$, then
\[ {\bf z}^*=\widetilde{\bf z}={\rm arg} \min_{{\bf z}\in \mathcal{T}\cap\mathcal{C}} f({\bf z}). \]

2) If $\widetilde{\bf z}\notin \mathcal{C}$, then there exists a ${\bf {z}}^*\in\mathcal{T}\cap\mathcal{C}_{edge}$ satisfying
\[ {\bf {z}}^*={\rm arg} \min_{{\bf z}\in \mathcal{T}\cap\mathcal{C}} f({\bf z}), \]
where $\mathcal{C}_{edge}$ denotes the boundary of $\mathcal{C}$.
\end{Lemma}

\begin{proof} Part 1) is obvious. In the following we  prove Part 2).

Let ${\bf \widehat{z}}\in\mathcal{T}\cap\mathcal{C}$ be finite and
\begin{equation} {\bf \widehat{z}}={\rm arg} \min_{\mathcal{T}\cap\mathcal{C}} f({\bf z}). \label{*}
\end{equation}
It is clear that Part 2) follows with ${\bf {z}}^*={\bf \widehat{z}}$ if
${\bf \widehat{z}}\in\mathcal{T}\cap\mathcal{C}_{edge}$.
Otherwise, suppose that
${\bf \widehat{z}}\in\mathcal{T}\cap\mathcal{C}_{int}$,  where $\mathcal{C}_{int}$ is the interior of $\mathcal{C}$.
 Note that $\widetilde {\bf z}\notin \mathcal{C}$, $\widetilde{\bf z}\in \mathcal{T}$ and
 ${\bf \widehat{z}}\in \mathcal{T}\cap\mathcal{C}_{int}$.
Therefore, there exists
${\bf {z}}^* \in\mathcal{T}\cap\mathcal{C}_{edge}$
such that for some $t\in(0,1)$, we have
\[ {\bf {z}}^*=(1-t) \widetilde{\bf z}+t{\bf \widehat{z}}\in \mathcal{T}\cap\mathcal{C}_{edge}. \]
Furthermore,
\[ f(\widetilde{\bf z})\leq f(\widehat{\bf z}). \]
Hence,
\[ %\label{n2}
f({\bf {z}}^*)\leq(1-t)f(\widetilde{\bf z})+t f({\bf \widehat{z}})\leq(1-t)f({\bf \widehat{z}})+tf({\bf \widehat{z}})
       =f({\bf \widehat{z}}),
\]
which together with (\ref{*}) yields that
\[ f({\bf {z}}^*)=f({\bf \widehat{z}}), \]
and thus,
\[ {\bf {z}^*}={\rm arg} \min_{{\bf z}\in \mathcal{T}\cap\mathcal{C}} f({\bf z}). \]
\end{proof}


\begin{Lemma}\label{lem*}
Assume that ${\bf b}\in \mathbb{R}^m$, $G\in \mathbb{R}^{m\times k}$,
and ${\rm rank} (G) =k$. Then the  solution  of the \emph{rank-k NLS} problem (\ref{n4}) is unique,
\end{Lemma}

\begin{proof} The proof is trivial and thus is omitted here.
\end{proof}

Now, we establish the recursive formula for the solution of \emph{rank-k NLS} problem (\ref{n4}).

\begin{theorem}\label{thm1}
Given ${\bf b}\in \mathbb{R}^m$, $G\in \mathbb{R}^{m\times k}$ and ${\bf g}_{k+1}\in \mathbb{R}^m$.
Assume that $G$ and and $\left[ \begin{array}{cc} G & {\bf g}_{k+1}\end{array}\right]$ are of full column rank.
Denote the unique solution  of the \emph{rank-k NLS} problem (\ref{n4}) by $s(G, {\bf b}) \in \mathbb{R}^k$.
Then the unique solution of the \emph{rank-(k+1) NLS} problem
\begin{eqnarray}\label{n5}
\left[ \begin{array}{c} {\bf y}^{\star} \\  y_{k+1}^{\star}\end{array}\right]= \arg
    \min_{{\bf y}\geq{\bf 0},y_{k+1}\geq0} \|(G{\bf y}+{\bf g}_{k+1}y_{k+1})-{\bf b}\|
\end{eqnarray} is given by
\begin{eqnarray*}
\begin{cases}
y_{k+1}^{\star}&=\frac{1}{\|{\bf g}_{k+1}\|^2}\big[{\bf g}^T_{k+1}\big({\bf b}-G\cdot
s(G-\frac{{\bf g}_{k+1}{\bf g}_{k+1}^T}{\|{\bf g}_{k+1}\|^2} G, {\bf b}-\frac{{\bf g}_{k+1} {\bf g}_{k+1}^T }{\|{\bf g}_{k+1}\|^2} {\bf b}))
\big]_+, \\
{\bf y}^{\star}&=s(G, {\bf b}-{\bf g}_{k+1}y^*_{k+1}).
\end{cases}
\end{eqnarray*}
\end{theorem}

\begin{proof}
We first consider the optimization problem
\begin{eqnarray}\label{n6}
\min_{{\bf y}\geq{\bf 0}} \|(G{\bf y}+{\bf g}_{k+1}y_{k+1})-{\bf b}\|.
\end{eqnarray}
Obviously, for any given ${\bf y}$, the solution $y_{k+1}$ to the problem \eqref{n6} is uniquely given by
\[ y_{k+1}=\frac{{\bf g}^T_{k+1}({\bf b}-G{\bf y})}{\|{\bf g}_{k+1}\|^2}.\]
So, the optimization problem \eqref{n6} reduces to
\begin{eqnarray}\label{n7}
\min_{{\bf y}\geq{\bf 0}} \|(G{\bf y}+{\bf g}_{k+1}\frac{{\bf g}^T_{k+1}({\bf b}-G{\bf y})}{\|{\bf g}_{k+1}\|^2})-{\bf b}\|
      =\min_{{\bf y}\geq{\bf 0}}\|\widetilde{G}{\bf y}-{\bf \widetilde{b}}\|,
\end{eqnarray}
where
\[ {\bf \widetilde{b}}={\bf b}-\frac{{\bf g}_{k+1}{\bf g}^T_{k+1}}{\|{\bf g}_{k+1}\|^2}{\bf b}, \quad
 \widetilde{G}=G-\frac{{\bf g}_{k+1}{\bf g}^T_{k+1}}{\|{\bf g}_{k+1}\|^2}G,
\]
and $\widetilde{G}$ is of full column rank.
The unique solution $\widetilde{\bf y}$ of the problem (\ref{n7}) is $s(\widetilde{G}, {\bf \widetilde{b}})$.
Therefore, the unique solution to the problem \eqref{n6} is given by
\begin{eqnarray*}
\widetilde y_{k+1} &=& \frac{{\bf g}^T_{k+1}({\bf b}-G\cdot s(\widetilde{G}, {\bf \widetilde{b}}))}{\|{\bf g}_{k+1}\|^2}, \\
\widetilde {\bf y} &=& s(G, {\bf b}-{\bf g}_{k+1} \widetilde y_{k+1}).
\end{eqnarray*}
Let
\[ \mathcal{T}:=\{ \left[ \begin{array}{c} {\bf y} \\ y_{k+1} \end{array}\right] |~{\bf y}\in \mathbb{R}^k, ~{\bf y}\geq0\}, \qquad
\mathcal{C}:=\{ \left[ \begin{array}{c} {\bf y} \\ y_{k+1} \end{array}\right] |~{\bf y}\in \mathbb{R}^k, ~{\bf y}\geq0, ~y_{k+1}\geq 0\}. \]
By Lemma \ref{lem0},
\begin{itemize}
\item if $\widetilde y_{k+1}\geq0$, then $\left[ \begin{array}{c} {\bf y}^{\star} \\  y_{k+1}^{\star}\end{array}\right]$ with
\begin{eqnarray*}
y^*_{k+1} &=& \widetilde y_{k+1} = \frac{{\bf g}^T_{k+1}({\bf b}-G\cdot s(\widetilde{G}, {\bf \widetilde{b}}))}{\|{\bf g}_{k+1}\|^2}
=\frac{[{\bf g}^T_{k+1}({\bf b}-G\cdot s(\widetilde{G}, {\bf \widetilde{b}}))]_+}{\|{\bf g}_{k+1}\|^2}, \\
{\bf y}^{\star} &=& \widetilde {\bf y} = s(G, {\bf b}-{\bf g}_{k+1} \widetilde y_{k+1})
   =s(G, {\bf b}-{\bf g}_{k+1} y^*_{k+1}),
\end{eqnarray*}
is the unique solution of the problem \eqref{n5};
\item if $\widetilde y_{k+1}<0$, then the unique solution $y_{k+1}$ of the problem  \eqref{n5} is
$$ y^{\star}_{k+1}=0=\frac{[{\bf g}^T_{k+1}({\bf b}-G\cdot s(\widetilde{G}, {\bf \widetilde{b}}))]_+}{\|{\bf g}_{k+1}\|^2}, $$
and consequently, the unique solution ${\bf y}$ of the problem \eqref{n5} is given by
\[ {\bf y}^{\star}=s(G, {\bf b}-{\bf g}_{k+1}y^*_{k+1}). \]
\end{itemize}

\end{proof}


Theorem \ref{thm1} can be used to derive the closed-form solution of the \emph{rank-k NLS} problem (\ref{n4}) for any integer $k\geq 1$.
As an example, we give the closed-form solutions of the \emph{rank-2 NLS} and \emph{rank-3 NLS} in the following two corollaries.

\begin{corollary}\label{cor1}
Assume that $G=\left[ \begin{array}{cc} {\bf g}_1 & {\bf g}_2\end{array}\right]\in \mathbb{R}^{m\times 2}$ is of full column rank.
Then the unique solution of the  \emph{rank-2 NLS} problem
\begin{align}\label{n10}
\left[ \begin{array}{c} y_1^* \\  y_2^*\end{array}\right]=\arg \min_{{\bf y}\geq0}\|G{\bf y}-{\bf b}\|=
{\rm arg} \min_{\{y_1,y_2\}\geq0}\|y_1{\bf g}_1+y_2{\bf g}_2-{\bf b}\|
\end{align}
is given by
\begin{eqnarray}\label{n9}
\begin{cases}
y_2^*&=\frac{1}{\|{\bf g}_2\|^2}\left[{\bf b}^T{\bf g}_2-{\bf g}^T_2{\bf g}_1
       \left[\frac{\|{\bf g}_2\|^2{\bf b}^T{\bf g}_1-{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1}{ \|{\bf g}_1\|^2\|{\bf g}_2\|^2
        -({\bf g}_1^T{\bf g}_2)^2  } \right]_{+}\right]_{+}\\
y_1^*&=\frac{1}{\|{\bf g}_1\|^2}[{\bf b}^T{\bf g}_1-({\bf g}^T_2{\bf g}_1)y_2^*]_{+}.
\end{cases}
\end{eqnarray}
\end{corollary}

\begin{proof}
Since  the solution of the \emph{rank-1 NLS} problem
\[ %\label{n11}
\min_{y_1\geq0}\|y_1{\bf g}_1-{\bf b}\|
\]
is given by
\[s({\bf g}_1, {\bf b})= \frac{[{\bf g}^T_1{\bf b}]_+}{\|{\bf g}_1\|^2}, \]
according to Theorem \ref{thm1}, the solution $y_2^*$ to \emph{rank-2 NLS} problem \eqref{n10} is
$$y^*_2=\frac{\big[{\bf g}^T_{2}({\bf b}-{\bf g}_1\cdot
s({\bf g}_1-\frac{{\bf g}_{2}{\bf g}^T_{2}}{\|{\bf g}_{2}\|^2}{\bf g}_1, {\bf b}-\frac{{\bf g}_{2}{\bf g}^T_{2}}{\|{\bf g}_{2}\|^2}{\bf b})\big]_+}{\|{\bf g}_{2}\|^2}.$$
Note that
\begin{eqnarray*}
s({\bf g}_1-\frac{{\bf g}_{2}{\bf g}^T_{2}}{\|{\bf g}_{2}\|^2}{\bf g}_1, {\bf b}-\frac{{\bf g}_{2}{\bf g}^T_{2}}{\|{\bf g}_{2}\|^2}{\bf b})
&=& \frac{\big[\big({\bf g}_1-{\bf g}_{2}\frac{{\bf g}^T_{2}{\bf g}_1}{\|{\bf g}_{2}\|^2}\big)^T\big({\bf b}-{\bf g}_{2}\frac{{\bf g}^T_{2}{\bf b}}{\|
{\bf g}_{2}\|^2}\big)\big]_+}{\left\|{\bf g}_1-{\bf g}_{2}\frac{{\bf g}^T_{2}{\bf g}_1}{\|{\bf g}_{2}\|^2}\right\|^2} \\
&=& \frac{\left[\|{\bf g}_2\|^2{\bf b}^T{\bf g}_1-{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1\right]_{+}}
{  \|{\bf g}_1\|^2\|{\bf g}_2\|^2-({\bf g}_1^T{\bf g}_2)^2 },
\end{eqnarray*}
then
\begin{eqnarray*}
\begin{cases}
y^*_2&=\frac{1}{\|{\bf g}_2\|^2}\left[{\bf b}^T{\bf g}_2-{\bf g}^T_2{\bf g}_1\left[\frac{\|{\bf g}_2\|^2{\bf b}^T{\bf g}_1
      -{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1}{ \|{\bf g}_1\|^2\|{\bf g}_2\|^2-({\bf g}_1^T{\bf g}_2)^2  }\right]_{+}\right]_{+}\\
y^*_1&=\frac{1}{\|{\bf g}_1\|^2}[{\bf b}^T{\bf g}_1-({\bf g}^T_2{\bf g}_1)y_2^*]_{+},
\end{cases}
\end{eqnarray*}
and (\ref{n10}) holds. \end{proof}

\begin{corollary}\label{cor2}
Assume that $G=\left[ \begin{array}{ccc} {\bf g}_1 & {\bf g}_2 &  {\bf g_3} \end{array}\right]\in \mathbb{R}^{m\times 3}$
is of full column rank. Then the unique solution of the \emph{rank-3 NLS} problem
\begin{align*}
  \left[ \begin{array}{c} y^*_1 \\ y^*_2 \\ y^*_3\end{array}\right]={\rm arg}
  \min_{{\bf y}\geq0}\|G{\bf y}-{\bf b}\|
 = {\rm arg} \min_{\{y_1,y_2,y_3\} \geq0}\|y_1{\bf g}_1+y_2{\bf g}_2+y_3{\bf g}_3-{\bf b}\|
\end{align*}
is given by \begin{align}\label{r3}
\begin{cases}
y^*_3&=\frac{1}{\|{\bf g}_3\|^2}[{\bf b}^T{\bf g}_3-({\bf g}^T_3{\bf g}_1)\widetilde{p}-({\bf g}^T_3{\bf g}_2)p]_{+}\\
y^*_2&=\frac{1}{\|{\bf g}_2\|^2}\left[{\bf b}^T{\bf g}_2-({\bf g}_3^T{\bf g}_2)y^*_3-{\bf g}^T_2{\bf g}_1\big[\frac{({\bf b}^T{\bf g}_1\|
                  {\bf g}_2\|^2-{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1)- ({\bf g}^T_3{\bf g}_1\|{\bf g}_2\|^2
                   -{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1)y^*_3}{\|{\bf g}_1\|^2\|{\bf g}_2\|^2-({\bf g}^T_2
                   {\bf g}_1)^2}\big]_{+}\right]_{+}\\
y^*_1&=\frac{1}{\|{\bf g}_1\|^2}[{\bf b}^T{\bf g}_1-({\bf g}^T_3{\bf g}_1)y^*_3-({\bf g}^T_2{\bf g}_1)y^*_2]_{+},
\end{cases}
\end{align}
where
\begin{eqnarray*}\label{q1}
p=\left[\frac{{\bf b}^T{\bf g}_2\cdot\|{\bf g}_3\|^2-{\bf b}^T{\bf g}_3\cdot{\bf g}^T_3{\bf g}_2}{\|{\bf g}_2\|^2\|{\bf g}_3\|^2
         -({\bf g}^T_3{\bf g}_2)^2}-\frac{{\bf g}^T_2{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_3{\bf g}_1}{\|
          {\bf g}_2\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)^2}\big[\frac{{\rm det}([{\bf b},{\bf g}_2,{\bf g}_3]^TG)}
           {{\rm det}(G^TG)}\big]_{+}\right]_{+},
\end{eqnarray*}
and
\begin{eqnarray*}\label{q2}
\widetilde{p}=\left[\frac{{\bf b}^T{\bf g}_1\cdot\|{\bf g}_3\|^2
                      -{\bf b}^T{\bf g}_3\cdot{\bf g}^T_3{\bf g}_1}{\|{\bf g}_1\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)^2}
                      -\frac{{\bf g}^T_2{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_3{\bf g}_1}{\|{\bf g}_1\|^2\|
                      {\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)^2}p\right]_{+}.
\end{eqnarray*}
\end{corollary}

\begin{proof}
Let
$${\bf \widehat{b}}={\bf b}-\frac{{\bf g}_{3}{\bf g}^T_{3}}{\|{\bf g}_{3}\|^2}{\bf b},~~
{\bf \widehat{g}}_1={\bf g}_{1}-\frac{{\bf g}_{3}{\bf g}^T_{3}}{\|{\bf g}_{3}\|^2}{\bf g}_{1},~~
{\bf \widehat{g}}_2={\bf g}_{2}-\frac{{\bf g}_{3}{\bf g}^T_{3}}{\|{\bf g}_{3}\|^2}{\bf g}_{2},~~
 $$
A simple calculation yields that
\begin{align}
{\bf \widehat{g}}^T_2{\bf \widehat{g}}_1
&=({\bf g}_{2}-\frac{{\bf g}^T_{3}{\bf g}_{2}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{1}
              -\frac{{\bf g}^T_{3}{\bf g}_{1}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{({\bf g}^T_2{\bf g}_1)\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)({\bf g}^T_3{\bf g}_1)}{\|{\bf g}_{3}\|^2},\label{n18}\\
\|{\bf \widehat{g}}_1\|^2
&=({\bf g}_{1}-\frac{{\bf g}^T_{3}{\bf g}_{1}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{1}
              -\frac{{\bf g}^T_{3}{\bf g}_{1}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{\|{\bf g}_1\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)^2}{\|{\bf g}_{3}\|^2},\label{n21}\\
\|{\bf \widehat{g}}_2\|^2
&=({\bf g}_{2}-\frac{{\bf g}^T_{3}{\bf g}_{2}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{2}
              -\frac{{\bf g}^T_{3}{\bf g}_{2}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{\|{\bf g}_2\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)^2}{\|{\bf g}_{3}\|^2},\label{n16}\\
{\bf \widehat{b}}^T{\bf \widehat{g}}_2
&=({\bf b}-\frac{{\bf g}^T_{3}{\bf b}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{2}
         -\frac{{\bf g}^T_{3}{\bf g}_{2}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{({\bf b}^T{\bf g}_2)\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)({\bf g}^T_3{\bf b})}{\|{\bf g}_{3}\|^2},\label{n17}\\
{\bf \widehat{b}}^T{\bf \widehat{g}}_1
&=({\bf b}-\frac{{\bf g}^T_{3}{\bf b}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})^T({\bf g}_{1}
          -\frac{{\bf g}^T_{3}{\bf g}_{1}}{\|{\bf g}_{3}\|^2}{\bf g}_{3})
=\frac{({\bf b}^T{\bf g}_1)\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)({\bf g}^T_3{\bf b})}{\|{\bf g}_{3}\|^2}.\label{n19}
\end{align}
Let $s(\left[ \begin{array}{cc} {\bf {\widehat g}}_1 & {\bf {\widehat g}}_2 \end{array}\right], {\bf {\widehat b}})
     =\left[
     \begin{array}{c}
          s_1(\left[ \begin{array}{cc} {\bf {\widehat g}}_1 & {\bf {\widehat g}}_2 \end{array}\right], {\bf {\widehat b}}) \\
          s_2(\left[ \begin{array}{cc} {\bf {\widehat g}}_1 & {\bf {\widehat g}}_2 \end{array}\right], {\bf {\widehat b}}) \\
     \end{array}
     \right]$
be the solution to the optimization problem
\[ \min_{y_1,y_2\geq0}\|y_1{\bf {\widehat g}}_1+y_2{\bf {\widehat g}}_2-{\bf {\widehat b}}\|. \]
Then from \eqref{n18}--\eqref{n19} and Corollary \ref{cor1}, we have
\begin{align*}
s_2(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})
&=\frac{1}{\|{\bf \widehat{g}}_2\|^2}\left[{\bf \widehat{b}}^T{\bf \widehat{g}}_2
             -{\bf \widehat{g}}^T_2{\bf \widehat{g}}_1\left[\frac{\|{\bf \widehat{g}}_2\|^2{\bf \widehat{b}}^T{\bf \widehat{g}}_1
             -{\bf \widehat{b}}^T{\bf \widehat{g}}_2\cdot{\bf \widehat{g}}^T_2{\bf \widehat{g}}_1}{\|{\bf \widehat{g}}_1\|^2\|{\bf \widehat{g}}_2\|^2-({\bf \widehat{g}}_1^T{\bf \widehat{g}}_2)^2}\right]_{+}\right]_{+}\nonumber\\
&=\left[\frac{{\bf b}^T{\bf g}_2\cdot\|{\bf g}_3\|^2-{\bf b}^T{\bf g}_3\cdot{\bf g}^T_3{\bf g}_2}{\|{\bf g}_2\|^2\|{\bf g}_3\|^2
             -({\bf g}^T_3{\bf g}_2)^2}-\frac{{\bf g}^T_2{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_3{\bf g}_1}
              {\|{\bf g}_2\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_2)^2}\big[\frac{{\rm det}([{\bf b},{\bf g}_2,{\bf g}_3]^TG)}
               {{\rm det}(G^TG)}\big]_{+}\right]_{+} \nonumber \\
&=p.
\end{align*}
Moreover,
\begin{eqnarray*}
s_1(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})
&=& \left[\frac{{\bf b}^T{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf b}^T{\bf g}_3\cdot{\bf g}^T_3{\bf g}_1}{\|{\bf g}_1\|^2\|{\bf g}_3\|^2
            -({\bf g}^T_3{\bf g}_1)^2}-\frac{{\bf g}^T_2{\bf g}_1\cdot\|{\bf g}_3\|^2-{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_3{\bf g}_1}
               {\|{\bf g}_1\|^2\|{\bf g}_3\|^2-({\bf g}^T_3{\bf g}_1)^2}
s_2(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right],
{\bf \widehat{b}})\right]_{+}\\
&=&\widetilde p.
\end{eqnarray*}
Therefore, according to Theorem \ref{thm1} and Corollary \ref{cor1}, the solution to the optimization problem
\[ \min_{y_1,y_2,y_3\geq0}\|y_1{\bf g}_1+y_2{\bf g}_2+y_3{\bf g}_3-{\bf b}\| \]
is
\begin{eqnarray*}
y^*_3 &=& \frac{1}{\|{\bf g}_{3}\|^2}\big[{\bf g}^T_{3}\big({\bf b}-[{\bf g}_1,{\bf g}_2]\cdot
s( \left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})\big)\big]_+ \\
%&=&\frac{1}{\|{\bf g}_{3}\|^2}\big[{\bf g}^T_{3}{\bf b}-{\bf g}^T_{3}{\bf g}_1\cdot
%s_1(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})
%-{\bf g}^T_{3}{\bf g}_2\cdot
%s_2(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})\big]_+,\\
&=&\frac{1}{\|{\bf g}_{3}\|^2}\big[{\bf g}^T_{3}{\bf b}-{\bf g}^T_{3}{\bf g}_1\cdot \widetilde{p}
-{\bf g}^T_{3}{\bf g}_2\cdot p\big]_+,
\end{eqnarray*}
with $s_1(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})=\widetilde{p}$, $s_2(\left[ \begin{array}{cc} {\bf \widehat{g}}_1 & {\bf \widehat{g}}_2\end{array}\right], {\bf \widehat{b}})=p$,
and
\begin{align*}
\begin{cases}
y^*_2&=s_2( \left[ \begin{array}{cc} {\bf g}_1 & {\bf g}_2 \end{array}\right],  {\bf b}-{\bf g}_{3}y^*_{3})\\
~&=\frac{1}{\|{\bf g}_2\|^2}\left[({\bf b}-{\bf g}_{3}y^*_{3})^T{\bf g}_2-{\bf g}^T_2{\bf g}_1\left[\frac{\|{\bf g}_2\|^2({\bf b}
       -{\bf g}_{3}y^*_{3})^T{\bf g}_1-({\bf b}-{\bf g}_{3}y^*_{3})^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1}{\|{\bf g}_1\|^2\|{\bf g}_2\|^2
       -({\bf g}^T_2{\bf g}_1)^2}\right]_{+}\right]_{+}\\
~&=\frac{1}{\|{\bf g}_2\|^2}\left[({\bf b}-{\bf g}_3y^*_3)^T{\bf g}_2-{\bf g}^T_2{\bf g}_1\big[\frac{({\bf b}^T{\bf g}_1\|{\bf g}_2\|^2
       -{\bf b}^T{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1)- ({\bf g}^T_3{\bf g}_1\|{\bf g}_2\|^2
       -{\bf g}^T_3{\bf g}_2\cdot{\bf g}^T_2{\bf g}_1)y^*_3}{\|{\bf g}_1\|^2\|{\bf g}_2\|^2
       -({\bf g}^T_2{\bf g}_1)^2}\big]_{+}\right]_{+}\\
y^*_1&=s_1(\left[ \begin{array}{cc} {\bf g}_1 & {\bf g}_2\end{array}\right], {\bf b}-{\bf g}_{3}y^*_{3})
=\frac{1}{\|{\bf g}_1\|^2}[({\bf b}-{\bf g}_{3}y^*_{3})^T{\bf g}_1-({\bf g}^T_2{\bf g}_1)y^*_2]_{+}.
\end{cases}
\end{align*}
Hence, Corollary \ref{cor2} is proved.
\end{proof}


